Multi-Channel Auction Design in the Autobidding World

Over the past few years, more and more Internet advertisers have started using automated bidding for optimizing their advertising campaigns. Such advertisers have an optimization goal (e.g. to maximize conversions), and some constraints (e.g. a budget or an upper bound on average cost per conversion), and the automated bidding system optimizes their auction bids on their behalf. Often, these advertisers participate on multiple advertising channels and try to optimize across these channels. A central question that remains unexplored is how automated bidding affects optimal auction design in the multi-channel setting. In this paper, we study the problem of setting auction reserve prices in the multi-channel setting. In particular, we shed light on the revenue implications of whether each channel optimizes its reserve price locally, or whether the channels optimize them globally to maximize total revenue. Motivated by practice, we consider two models: one in which the channels have full freedom to set reserve prices, and another in which the channels have to respect floor prices set by the publisher. We show that in the first model, welfare and revenue loss from local optimization is bounded by a function of the advertisers' inputs, but is independent of the number of channels and bidders. In stark contrast, we show that the revenue from local optimization could be arbitrarily smaller than those from global optimization in the second model.

==> multi_channel (1)/01-intro.tex <==
\section{Introduction}

Advertisers are increasingly using automated bidding in order to set bids for ad auctions in online advertising. Automated bidding simplifies the bidding process for advertisers -- it allows an advertiser to specify a high-level goal and one or more constraints, and optimizes their auction bids on their behalf~\cite{googlebiddingpage,metabiddingpage,tiktokbiddingpage,twitterbiddingpage}. A common goal is to maximize conversions or conversion value. Some common constraints include Budgets and TargetCPA (i.e. an upper bound on average cost per conversion). 
This trend has led to interesting new questions on auction design in the presence of automated bidders~\cite{AggarwalBM19,DengMMZ21,BalseiroDMMZ21,balseiro2021robust}. 

One central question that remains unexplored is how automated bidding affects optimal auction design in the {\em multi-channel setting}. 
%that is motivated by practice but has received relatively sparse attention in the auto-bidding literature. Specifically, 
It is common for advertisers to show ads on multiple channels and optimize across channels. 
For example, an advertiser can optimize across Google Ads inventory (YouTube, Display, Search, Discover, Gmail, and Maps) with Performance Ads~\cite{googlemaxperformance}, or can optimize across Facebook, Instagram and Messenger with Automated Ad Placement~\cite{metaadplacement}, or an app developer can advertise across Google's properties including Search, Google Play and YouTube with App campaigns~\cite{googleuniversalappcampaigns}. With traditional quasi-linear bidders, the problem of auction design on each channel is independent of other channels' designs. However, when advertisers use automated bidders and optimize across channels, the auction design of one channel creates externalities for the other channels through the constraints of automated bidders.

Motivated by this, we introduce the problem of auction design in the multi-channel setting with automated bidding across channels. In particular, we study the problem of setting reserve prices across channels. We consider two behavior models: {\em Local} and {\em Global}. In the {\em Local} model, each channel optimizes its reserve price to maximize its own revenue, while in the {\em Global} model, the channels optimize their reserve prices {\em globally} in order to maximize the total revenue across channels. The main question is: {\em what is the revenue loss from optimizing {\em locally}, rather than {\em globally}}? 

We consider this question in two settings: one in which each channel has full control over its reserve prices, and one in which the channels have to respect an externally-imposed lower bound on the reserve prices. The first setting which we call {\em Without Publisher Reserves} is very common in practice and arises when the impressions are owned by the selling channel, or when the publisher leaves the pricing decisions to the selling channel. The second setting which we call {\em With Publisher Reserves} arises when the impressions are owned by a third-party publisher that sets a floor price for its impressions -- this could come from an outside option for selling the impression. This is common in Display advertising where the selling channel is often different from the publisher who owns the impressions.
%and shed light on the 
%revenue implications of whether each channel optimizes its reserve prices {\em locally}, or whether the channels optimize them {\em globally} to maximize total revenue. 

{\bf Model:}
Our model consists of $k$ channels, each selling a set of impressions. Each channel can set a uniform reserve price. The uniform reserve price is in the cost-per-unit-value space\footnote{See Section~\ref{sec: further-discussions} for a discussion of uniform reserve prices in the cost-per-impression space} (see Section~\ref{subsec:bidders} for details). This is motivated by the observation that, in practice, values are commonly known by the channels; values are usually click-through-rate or conversion-rate of an ad, as in~\cite{AggarwalBM19}, and the channels have good estimates for those. Besides the reserve prices set by channels, in the {\em With Publisher Reserves} setting, each impression could have a price floor set by the publisher who owns the impression.
Each impression is sold in a Second-Price-Auction with a floor price that depends on the reserve price set by the selling channel and the price constraint set by the publisher. Bidders want to maximize their conversions (or some other form of value) subject to one of two types of constraints: (1) Budget, an upper bound on spend and (2) TargetCPA, an upper bound on the average cost per conversion. The model also allows standard quasi-linear bidders with no constraints.
The game consists of two main stages: First, each channel simultaneously announces its reserve price; then, bidders bid optimally for the different impressions. 

\subsection{Our results}
The paper's main focus is to compare the revenue\footnote{See Section~\ref{sec: further-discussions} for a brief discussion of {\em welfare}} at equilibrium when channels optimize locally, i.e. each sets its reserve price(s) to maximize its own revenue, to the revenue where channels act globally and set their reserve prices to maximize the sum of the total revenue.
%\footnote{A more general version of the model would include coalitions so that channels belonging to the same coalition set reserve prices to maximize the total revenue of the respective coalition.\apnote{Shall we add this here?} \ganote{we can leave it here for now, can worry about it later}}
We define the Price of Anarchy (PoA) as the worst-case ratio between the total revenue when the channels optimize locally compared to the case where the channels optimize globally. Our main goal is to bound the Price of Anarchy in the two settings: {\em Without Publisher Reserves}, and {\em With Publisher Reserves}.

%\Junyao{Maybe we can talk about $PoA=0$ in the most general setting, which is why we focus on the following important setting and later the scaled channels; the order of the results in intro do not have to follow the order of the technical sections}\ganote{That is the order we originally had in the abstract. I feel that saying poa=0 first makes this one appear like a less important setting}\Junyao{ok, then we should emphasize this setting is important}\ganote{agreed. we can add a phrase saying that this is a common setting}\Junyao{agree}
\subsection*{Setting without Publisher Reserves}
In order to bound the Price of Anarchy, we first bound the local and global revenue in terms of the optimal Liquid Welfare 
%\Andres{the highest possible revenue all channels can possibly obtain} 
(see Section~\ref{sec:model} for the definition). These revenue bounds are interesting in their own right and the proof methodology gives (non-polytime) algorithms for determining good reserve prices. 

We first consider the worst-case revenue in the local model where each channel is optimizing for its own revenue, compared to the optimal Liquid Welfare. We show in Theorem~\ref{thm:rev-local} that the worst-case revenue is at least $\Omega(\frac{1}{\log \eta})$ 
fraction of the optimal Liquid Welfare, where $\eta$ depends on the bidders' inputs\footnote{$\eta$ is the maximum of the ratio of the highest to lowest TargetCPA among TargetCPA bidders and a ratio defined (in Definition~\ref{def:budget-fraction}) for Budgeted bidders.} and quantifies the heterogeneity of the pool of bidders. This lower bound on revenue trivially carries over to the setting where the channels are optimizing globally and to the single-channel setting. Next, we show that this bound is tight up to constant factors (Proposition~\ref{ex:revg-ub}). In particular, we give an example in the single-channel setting where the optimal revenue with a uniform reserve price is $O(\frac{1}{\log \eta})$ of the optimal Liquid Welfare. This upper bound also applies to the global and local models in the multi-channel setting. In other words, the upper bound and lower bounds on the gap between Liquid Welfare and revenue in each of these settings is $\Theta(\log \eta)$. That naturally makes one wonder: Is optimizing locally as good for revenue as optimizing globally? If we look into the gap bounds, we find that they arise from trying to capture values of different scales with a uniform reserve price. And one might conjecture that since the source of the gap applies to both the global and local model, that even if there is a revenue gap between the two models, it should depend on different factors. Surprisingly, we show that the gap between optimizing locally and globally is exactly the same $\log \eta$ factor (Theorem~\ref{lem:tight-PoA}).
%We show a lower bound on total revenue that depends logarithmically on the ratio between the highest and lowest target $\tcpa$ and a similar ratio defined for Budgeted bidders in both the local and the global setting. This gives us an identical lower bound for PoA. These bounds are nearly tight as shown in Examples~\ref{ex:revg-ub} and~\ref{}.
Note that in all the above settings, the revenue guarantee is independent of the number of channels and bidders and depends only on the heterogeneity of the bidders.

\subsection*{Setting with Publisher Reserves}
In stark contrast to the setting without publisher reserves, we show that the PoA in this setting can be arbitrarily small even with one $\tcpa$ bidder (Theorem~\ref{th:general-publisher-model}). The gap example depends heavily on the asymmetry between the different channels. Motivated by this, we consider the restricted setting where each channel sells a random sample of the impressions (see Section~\ref{publisher-reserve} for the exact details). For this case, with one $\tcpa$ bidder in the game, we show that under some mild constraint on the channels' strategies, the PoA = $1/k$, where $k$ is the number of channels. 
%{\color{red}Moreover, we show that for this one-bidder game, the equilibrium is unique and can be computed using a simple algorithm.}\Andres{not correct. we don't have this result.}\ganote{because of the lack of upper bound on reserve?}\andres{yes, to hold our algo we need to restrict channels to set reserve less than the target. This may be suboptimal. What is true, though is that for any pure strat eq PoA=1/k (it may fail to exists though).} \ganote{Yeah. have we added the proof and the algo to the paper? for the restricted case?}\Andres{No for the paper, we don't have the restricted setting.} \ganote{then we can remove it from here.}\Andres{agree}.
%\ganote{Usually the POA is > 1. Price is large means that not having coordination leads to a large price to pay. Would it be a lot of work to say it like that?}\Andres{let me ask junyao who rewrote sect 5.}\ganote{it's not too important... we can also change for the camera ready}\Andres{maybe better for camera ready we may have typos by changing it now.}\ganote{sg}\Junyao{https://arxiv.org/pdf/1607.07684.pdf we should listen to the guys who defined it}
When the channels optimize globally, the equilibrium is efficient and all channels set low reserve prices. On the other hand, for the equilibrium in the local optimization model, the larger channels (in terms of the volume of impressions they own) set low reserve prices while small channels are extractive and set high reserve prices.   


\subsection*{Hardness of Equilibrium Computation}
To complement our Price of Anarchy results, we also study
the computational complexity of computing the equilibrium of the game. 
We show an impossibility result -- that it is $\PPAD$-hard to compute the subgame equilibrium of the bidders (Theorem~\ref{thm:subgame-hardness}). To prove this result, we use gadget reduction from the problem of finding approximate Nash equilibrium for $0$-$1$ bimatrix game, and we need to handle many difficulties unique to our subgame, which we explain with more details in Section~\ref{sec:hardness} and Appendix~\ref{app:proof-of-hardness}.

\subsection*{Key implications of our results}
Our results have several implications for setting reserve prices in the multi-channel setting: 
\begin{itemize}
    \item The revenue gap between local and global optimization depends heavily on whether there are publisher-imposed reserve prices. 
    \item Without publisher reserves, the worst-case gap between the revenue in the local model and the global model is $\Theta(\log \eta)$, where $\eta$ captures the heterogeneity of the bidders' inputs and is independent of the number of channels and bidders. Thus it is better to optimize globally when possible. %This is true even though the revenue in each model can be $\Theta(\log \eta)$ away from the optimal liquid welfare.
    \item Without publisher reserves, it is possible to obtain a revenue of $\Theta(\frac{1}{\log \eta})$ fraction of the optimal Liquid Welfare by setting uniform reserve prices. This observation is not surprising in the single-channel setting and for global optimization in the multi-channel setting, but it is remarkable that it holds even with local optimization, where the selfishness of a channel could have made it difficult for other channels to make revenue. We also note that the approximation can be improved by setting reserve prices at a more granular level, rather than a uniform reserve price. In that case, the approximation ratio will depend on the heterogeneity of bidders per slice.
    \item With publisher reserves, the gap between the revenue in the local and global model can be arbitrarily large. This can happen even when only one of the channels has external pricing constraint.
\end{itemize}

\subsection*{Organization of the paper}
We present a formal model of the problem in Section~\ref{sec:model}. Then, in Section~\ref{sec:hardness}, we show that it is $\PPAD$-hard to compute the equilibrium of the sub-game. In Section~\ref{zero-publisher-reserve}, we study the setting without publisher reserves and present a tight bound on the Price of Anarchy, as well as on the gap between the revenue and optimal Liquid Welfare in the local and global models. In Section~\ref{publisher-reserve}, we study the setting with publisher reserves and show the Price of Anarchy is 0. We also study a restricted version of this setting, and show a Price of Anarchy of $1/k$ for that version. Finally, in Section~\ref{sec: further-discussions}, we discuss extensions for welfare and for setting reserve prices in the cost-per-impression space.

\begin{comment}

\ganote{we have to cite these in the intro to make it clear that we are not exposing anything new or particular to google}
Autobidding under constraints

The Landscape of Auto-bidding Auctions: Value versus Utility Maximization

Towards Efficient Auctions in an Auto-bidding World

Google Ads Help Center: About automated bidding. https://support.google.com/google-ads/answer/2979071?hl=en

Tiktok Business Help Center: About App Event Optimization. https://ads.tiktok.com/help/article?aid=179845248081724490

Your Guide to Meta Bid Strategies. https://www.facebook.com/business/m/one-sheeters/facebook-bid-strategy-guide

https://forecasts-na1.emarketer.com/584b26021403070290f93a55/5851918a0626310a2c186aad

---old intro---
Over the past years, an important trend in the Ad-auction ecosystem is that advertisers have increasingly started to adopt autobidding mechanisms to bid for impressions. Part of the explanation of this adoption has grounds that most autobidding mechanisms are suitable for situations where advertisers face constraints on the price they have to pay for the impressions (for example, budget constraints or average cost per acquisition constraints). These constraint advertisers face an important challenge when bidding among different channels\apnote{channels?} which frequently happens in practice. Likewise, each channel faces a similar problem when optimizing their auctions as it generates externalities on the other channels due to the constraint advertisers. 

This paper sheds light on this multi-channel problem by comparing the revenue 
%and welfare 
implications when each channel {\em locally} optimizes its auctions versus the case where channels {\em cooperate} to design their auctions to maximize the aggregated revenue. We show that from the channels' perspective, the revenue-loss by acting locally can be arbitrarily large compared to the case where they cooperate. Our results depend, though, on the pricing constraint that publishers could set on the impressions they own. When publishers do not set any pricing constraint, there is a constant factor gap between the local revenue and the (optimal) cooperative revenue.   

\section{Notes:}

\begin{itemize}
    \item Frame the setting from the point of view of a bidder who has constraints across all the channels they are bidding on. E.g. tcpa constraint, budget constraint.
    \item The channels could either co-ordinate or not (to begin with, either all co-ordinate or all are local -- can leave the mixed problem as an open problem)
    \item Questions: how does the welfare of the bidders and the revenue of the channels change with cooperation or not. 
    \item For multiple tcpa bidders, only consider self-sourced prices. Show that can get revenue at least 1/log maxtcpa/mintcpa (clarify the model as to what is public and what is private) fraction of the optimal welfare. Hence also showing same bound for welfare for the channel-chosen reserve price (if the reserve prices were zero, then we know that we get a welfare of 1/2 for our WINE paper, but here we are letting the channels locally choose their reserve prices to maximize their revenue, which could lead to a lower welfare). This applies to multiple channels as well, both for co-ordinated case and local case. Open question: Is there an instance where the revenue in the local case is log away from the revenue in the co-ordinated case (same question for welfare)? Also $\PPAD$ hardness. 
    \item For multiple tcpa and multiple budgeted bidders, we can show for one channel, a bound of log for revenue and welfare wrt the optimal welfare. But for multiple channels, we still need to extend.
    \item Next, we add exogenous (publisher-sourced) prices to the model which serve as a lower bound on the price of any given query. And we ask the same question. For the one tcpa case, we show a POA of 1/k, in contrast to the setting without exogenous prices. (We assume that reserve is below t -- how do we justify?) Can we extend the POA to the multiple tcpa case -- it will have to be worse than 1/k and 1/log max/min. Is there an example that shows 1/k log max/min e.g. (this is of course only if we get the example of 1/log without exogenous prices).
\end{itemize}

---older intro----



Large-scale online channels typically contain multiple channels in which advertisers participate in the respective ad-auctions to buy impressions. In each of these channels, channels spend high resources trying optimize the specific auction systems. This localized optimization, at the channel level, is usually explained because of the idiosyncratic differences of the auction systems across the channels and by the synchronization cost of having a unified policy for the different channels. In this paper, we quantify the channel's value of synchronizing the different channels in tuning the auction system across channels.

To quantify this value of synchronization, we depart from the standard profit-maximizer framework and consider advertisers bidding through an automated system. As discussed in \cite{AggarwalBM19}, this modelling assumption goes in line with the increasing adoption autobidding systems by advertisers. In particular, our paper focus on two of the most common autobidding formats: the $\tcpa$ format that consists in maximizing the volume of impressions given a target cost per action constraint reported by the advertiser;{\color{red} and the budget constraint format consisting in maximizing value given a budget constraint reported by the advertiser. }  

Our model consists of one channel owning multiple channels. Each channel each owns a fraction of the total set of impressions that are sold using a Second Price Auction with a reserve price chosen by the channel. There are multiple advertisers bidding for each of the impressions in each of the auctions. Following the previous paragraph, we assume that advertisers' marginal bid in each of the auction system is selected to maximize the aggregated value of impressions (among all channels) with the restriction to either meet a $\tcpa$ constraint {\color{red} or a budget constraint}. In this framework, we study the {\em Price of Synchronization (POSc)}: the aggregated channel's revenue when each channels sets reserve price to maximize their respective revenue compared to the optimal case where reserve price are selected to maximize the aggregated revenue.    




We start our analysis by considering a simplified version of the general case that considers a single $\tcpa$ bidder facing a price-landscape. We distinguish two micro-foundation of the price-landscape leading to different POSc. When the price-landscape comes from bids of other quasi-linear (ql) bidders bidding in each impression (the ql-bidders do not face any constraint) we show that in the (generically) unique equilibrium the POSc is constant independent of how many channels the channel owns.\footnote{The equilibrium depends on a restriction on the reserve prices the channel can set. More precisely, we impose that each channels cannot set a a reserve price greater than $T$ (cannot be fully extractive channel).} As part of the analysis, we provide a simple algorithm that computes the equilibrium. In the second micro-foundation for the price-landscape, we assume that the price comes from a restriction set by the publishers owning the impressions. In the second model, we show that in the
(generically) unique equilibrium the POSc= $\frac 1 k$, where $k$ corresponds to the number of channels the plaftorm owns. We also provide an algorithm that computes the equilibrium. \apnote{We should discuss about where the inefficiency comes: that big channels subsidizing small channels} \apnote{Discuss the implications of the result: for ql-bidders the benefit of cooperating on different channels in the channel is second order magnitude and would be outweighed by the normal costs of synchronizing the different channels. In  the publisher sourced setting where each publisher set a minimum price for the query to be sold we show that POA linearly depends on the channels the channel owns.}

We next present the general model where there are multiple $\tcpa$ advertisers bidding in the different channels. In contrast with the one $\tcpa$ bidder reduced form model, we show that a simple characterization of the equilibrium cannot exists. More precisely, we show that computing an equilibrium for the channels (and in particular the subgame equilibrium for the bidders) is $\PPAD$-hard. We bypass this technical challenge, and provide an algorithm that sets reserve prices for each channel that provide a constant factor of the liquid welfare. Using this algorithm, we show that POSc is independent of the number of channels the channel owns and is logarithmicly dependent on the TCPA constraint. \apnote{(i) Do we have an existence result of equilibrium? (ii) Is the PoA tight?).}


Our first result, is a complexity impossibility result showing that an analytical solution for the general is not possible. Similar to \cite{CKSM18} that shows a hardness result to compute an equilibrium for profit-maximizing bidder with budget constraint we show that finding an equilibrium for multiple $\tcpa$ bidders is $\PPAD$-hard.

Given the above impossibility result, we introduce a reduced form that considers a single $\tcpa$ bidder bidding competing with quasi-linear (ql) bidders for each impression (the ql-bidders do not face any constraint). Our first result presents the (generically) unique equilibrium between the channels and provide a simple algorithm to compute it.\footnote{The equilibrium depends on a restriction on the reserve prices the channel can set. More precisely, we impose that each channels cannot set a a reserve price greater than $T$ (cannot be fully extractive channel).}We show that the POSc is constant independent of how many channels the channel owns.

We next consider the general model where there are multiple TCPA advertisers bidding in the different channels. In contrast with the one TCPA bidder model, we show that a simple characterization of the equilibrium cannot exists. More precisely, we show that computing an equilibrium for the channels (and also the bidding equilibrium for the TCPA-bidders) is $\PPAD$-hard. Still, even without having a characterization of the equilibrium, we are able to compute a bound for POA ({\color{red}Andres:  (i) Do we have an existence result of equilibrium? (ii) Is the PoA tight?}). Our bound is independent of the number of channels the channel owns and is logarithmicly dependent on the TCPA constraint. 


The first set of results presented in the paper suggest that the benefit of coordinating the different channels in the channel is second order magnitude and would be outweighed by the normal costs of synchronizing the different channels. We shed caution on this conclusion, by showing that the previous results critically depend on the specifics of the ad exchange. For example, in a publisher sourced setting where each publisher set a minimum price for the query to be sold we show that POA linearly depends on the channels the channel owns. We consider a simplified setting with one TCPA bidder and price landscape chosen by the publisher. In this scenario, we characterize the (generically) unique equilibrium for the channels' game and provide a simple algorithm to compute it. We then obtain the POA and show that it's value is $\frac 1 k$, where $k$ corresponds to the amount of channels the plaftorm owns. 

\end{comment}

==> multi_channel (1)/011-related.tex <==
\section{Related Work}
\medskip
\noindent {\bf Autobidding.} There has been a lot of recent interest in exploring questions related to automated bidding, including bidding algorithms and their equilibria~\cite{AggarwalBM19}, and auction design in the presence of automated bidding~\cite{DengMMZ21,BalseiroDMMZ21,balseiro2021robust}. \citet{AggarwalBM19} initiate the study of autobidding and find optimal bidding strategies for a general class of autobidding constraints. They also prove the existence of an equilibrium and prove a lower bound on liquid welfare at equilibrium compared to the optimal liquid welfare. \citet{DengMMZ21} show how boosts can be used to improve welfare guarantees when bidders can have both TargetCPA and Budget constraints, potentially at the cost of revenue. \citet{BalseiroDMMZ21} characterize the revenue-optimal single-stage auctions with either value-maximizers or utility-maximizers with TargetCPA constraints, when either the values and/or the targets are private. Similar to our paper, \citet{balseiro2021robust} also study reserve prices in the presence of autobidders, and show that with TargetCPA and Quasi-linear bidders, revenue and welfare can be increased by using (bidder-specific) reserve prices. They do not study budget-constrained bidders.
%Besides the model of constrained optimization, there is another generalization of the utility models with ROI constraints adopted by Babaio et al. [2021], Goel et al. [2014, 2019]. In particular, the negative payment term in the utility function is replaced by a
% general cost, which is often a convex function of the payment.
%study the auction design problem of selling an item to bidders with TargetCPA constraint, with either utility maximization or value maximization as their objective, and with either the values or targets as private. They give optimal mechanisms for each setting. This paper does not consider budget-constrained bidders. \citet{DengMMZ21}, the authors study the problem of designing mechanisms for TargetCPA and Budget-constrained bidders with the objective of increasing liquid welfare, potentially at the cost of revenue.
All of the above papers are in the single channel setting. \medskip

\noindent {\bf Auction design with multiple channels.}
Most of this stream of literature have focused on models where multiple channels (auctioneers) compete to take captive profit-maximizers buyers \cite{Burguet1999ImperfectCI, ellison, preston}. The competition across channels leads to lower reserve prices, obtaining lower revenues and more efficient outcomes~\cite{virag}. Our model differs from them in that our bidders are not captive but are instead are optimizing under their autobidding constraints. Interestingly, we show that in some cases the competition among channels leads to higher reserve prices, and at the same time, improves welfare (see Theorem~\ref{th: scaled channels PoA=0}.).
%\ganote{we don't have the improve welfare part}%\Andres{just add a discussion about it. The result is in the appendix. We can remove it (especially if we remove the discussion i just added.)}


%\citet{Burguet1999ImperfectCI} 
%For multi-channel auction design, ~\cite{Burguet1999ImperfectCI} study the problem of setting reserve prices when two channels are each trying to sell an identical good to a pool of unit-demand buyers.

\begin{comment}

quote from robust auction design paper (https://arxiv.org/pdf/2111.02468.pdf) we can use

"While there have been recent work addressing this problem, most previous studies have
several shortcomings, e.g., they reduce such eciency loss by introducing boosts that explicitly or implicitly
rely on the accurate knowledge of the advertiser values [Deng et al., 2021b], or they aim to optimize for either
value-maximizing buyers or utility maximizing buyers (and not a mixture of auto-bidders) [Balseiro et al., 2021a],
or they aim to optimize only welfare and not revenue [Deng et al., 2021b]."


Another reference: Pai and Vohra, Optimal auctions with financially constrained buyers, 
https://users.nber.org/~confer/2010/MDf10/Pai_Vohra.pdf
Optimal mechanism for budgeted utility maximizers in a very constrained setting, priors, single good, etc.


\end{comment}

==> multi_channel (1)/02-model.tex <==
\section{Model}
\label{sec:model}
Our baseline model considers a set of bidders (advertisers) $J$ interested in purchasing a set of impressions $I$ that are sold by $K$ different channels.
The impressions that channel $k$ sells, $i\in I_k$, are sold using a second-price auction with a floor price. This floor price depends on the reserve price $r_k$ chosen by the channel and by the minimum price $p_{i}$ set by the publisher that owns the impression\footnote{The publisher might have an outside option to sell some of the impressions and sets a reserve price to account for that. These reserve prices are prechosen by the publishers and hence are fixed constants known to both channels and bidders.}.

\subsection{Bidders}
\label{subsec:bidders}
Motivated by the most common bidding formats that are used in practice, we assume that each bidder can be one of the following types: a {\em $\tcpa$} bidder, a {\em $\budgeted$} bidder, or a {\em Quasi-linear ($\ql$)} bidder. We denote by $J_{\tiny \tcpa}$, $J_{\tiny \budgeted}$ and $J_{\tiny \ql}$ the set of bidders that are $\tcpa$, $\budgeted$ and $\ql$ bidders, respectively.
 
Each Bidder $j$ has a value (e.g. conversion rate) $v_{j,i}$ for impression $i$ and submits a bid $b_{j,i}$ for the impression. A bidder's cost for buying impression $i\in I_k$ is 
\begin{align}
    & c_{j,i}(\b_{i},\r) = \max\{\max_{\ell\neq j\textrm{ s.t. } b_{\ell,i}\ge\max\{r_k v_{\ell,i},\,p_{i} v_{\ell,i}\}}\{ b_{\ell,i}\},\,r_k v_{j,i},\,p_{i} v_{j,i}\} \label{con:c},
\end{align}
where $\b_{i} = (b_{j,i})_{j\in J}$ (note we use the notation $c_{j,i}(\b_{i},\r)$ for simplicity, even though $c_{j,i}(\b_{i},\r)$ does not depend on $b_{j,i}$) and $\r=(r_k)_{k\in K}$ (because $p_i$'s are fixed constants prechosen by the publishers, for simplicity we do not include them as variables). That is, a bidder's cost for an impression is the maximum among (i) the bids of the bidders who bid above their own reserve prices, (ii) reserve price set by the channel which owns the impression, and (iii) reserve price set by the publisher. Also, note that the reserve prices $r_k$ and $p_i$ are multiplied by $v_{j,i}$ to get the final floor price of impression $i$ for bidder $j$. In other words, the reserve prices are in the cost-per-unit-value space. We will refer to the final reserve price of impression $i$ for bidder $j$ by $r_{j,i}:=\max\{r_k v_{j,i},\,p_{i} v_{j,i}\}$. Now we explain the bidder types.

\begin{comment}
Furthermore, we define a lower bound of bidder's cost for buying impression $i\in I_k$ which will be useful later:
\begin{align}
    & c_{j,i}^{(\lb)}(\b_{i}) = \max\{\max\{ b_{m,i} \mid m\neq j,\, b_{m,i}<\max\{r_k,p_i\} v_{m,i}\},\, r_k v_{j,i},\, p_{i} v_{j,i}\} \label{con:c_lb},
\end{align}
where the first term inside the top-level maximum operator is the maximum of the bids of all the bidders who bid strictly below their reserve prices (note these bidders will not get the impression $i$, but their bids play the role like reserve prices).
\end{comment}

\smallskip
{\bf $\ql$ bidder:} This is a traditional profit-maximizing bidder with no constraint. 
The dominant strategy for such a Bidder $j$ is to bid her value $v_{j,i}$ for impression $i$, regardless of how everyone else bids for that impression.

\medskip

{\bf $\tcpa$ bidder:} Such Bidder $j$ maximizes the number of conversions (i.e., the total value of the impressions which the bidder gets) subject to the constraint that the average cost per conversion is no greater than their $\tcpa$ $T_j\ge 0$. Namely, bidder $j$ solves the following maximization problem:
\begin{align}
    \max_{\forall i\in I,\, b_{j,i}\ge0,\,x_{j,i}\in[0,1]} \quad &  \sum_{i\in I \textrm{ s.t. } b_{j,i}\ge c_{j,i}(\b_{i},\r)} v_{j,i}x_{j,i}\nonumber\\
    \mbox{s.t. }\quad & \sum_{i\in I} c_{j,i}(\b_{i},\r) x_{j,i} \leq T_j \cdot \sum_{i\in I} v_{j,i} x_{j,i}\quad\forall j\in J\nonumber\\
    & x_{j,i} = 1 \mbox{ if } b_{j,i} > c_{j,i}(\b_{i},\r)\quad\forall j\in J,i\in I\label{con:x}.
\end{align}
\medskip

{\bf $\budgeted$ bidder:} Such Bidder $j$ maximizes the number of conversions subject to a budget constraint $B_j$. Namely, Bidder $j$ solves the following maximization problem:
\begin{align}
    \max_{\forall i\in I,\, b_{j,i}\ge0,\,x_{j,i}\in[0,1]} \quad &  \sum_{i\in I \textrm{ s.t. } b_{j,i}\ge c_{j,i}(\b_{i},\r)} v_{j,i}x_{j,i}\nonumber\\
    \mbox{s.t. }\quad & \sum_{i\in I} c_{j,i}(\b_{i},\r) x_{j,i} \leq B_j\quad\forall j\in J\nonumber\\
    & x_{j,i} = 1 \mbox{ if } b_{j,i} > c_{j,i}(\b_{i},\r)\quad\forall j\in J,i\in I\label{con:x1}.
\end{align}
\medskip

Notice that both $\tcpa$ bidder and $\budgeted$ bidder are allowed to decide the fraction of an impression they get in case they are tied for that impression (we say that bidder $j$ is {\bf tied} for an impression $i$ if $b_{j,i}=c_{j,i}(\b_i,\r)$). This is in line with the standard approach in the literature (e.g., budget pacing equilibrium~\cite{conitzer2021multiplicative}) that endogenizes the tie-breaking rule as part of the equilibrium concept which we will define shortly. Moreover, in the following proposition, we show that given other bidders' bids, it is optimal for a $\tcpa$ bidder (or a $\budgeted$ bidder) $j$ to bid uniformly\footnote{Qualitatively, this is same as the well-known result of~\citet{AggarwalBM19}. They prove this by introducing small perturbations to bidders' values. Instead, we take the approach that endogenizes the tie-breaking rule as part of the equilibrium concept, which is the standard approach in the literature for proving existence and computational complexity of equilibrium.}, i.e., the bids are characterized by a single {\bf bidding parameter} $\alpha_j\ge 0$ as follows: $\forall i\in I,\,b_{j,i}=\alpha_jv_{j,i}$.

\begin{proposition}\label{prop:uniform_bidding_optimal}
For a $\tcpa$ bidder (or a $\budgeted$ bidder resp.) $j$, the optimal bids for Problem~\eqref{con:x} (or~\eqref{con:x1} resp.) have the following form: there exists $\alpha_j\ge 0$ such that $\forall i\in I,\,b_{j,i}=\alpha_jv_{j,i}$.
\end{proposition}
The proof of Proposition~\ref{prop:uniform_bidding_optimal} is provided in appendix.

\subsection{Bidders' Subgame}

Bidders observe the reserve prices $\r = (r_k)_{k\in K}$ posted by the channels and decide their bids $\b_i(\r)$ for each impression $i$, and if a Bidder $j$ is tied for impression $i$, they can also decide the fraction $x_{j,i}(\r)$ of impression $i$ they get. In the previous subsection, we have shown that for any bidder of any type, the best response given other bidders' bids is bidding uniformly, and hence, we assume that each bidder $j$ uses uniform bidding with a bidding parameter $\alpha_j(\r)$.

Moreover, we assume that in the bidders' subgame, bidders use the {\em undominated uniform} bidding strategies. Specifically, for a $\ql$ bidder, bidding less than their value is dominated by bidding their value, and for a $\tcpa$ bidder $j$, using a bidding parameter less than $T_j$ is dominated by using a bidding parameter $\alpha_j(\r)=T_j$. To see the latter, notice that a $\tcpa$ bidder $j$ using a bidding parameter strictly less than $T_j$ cannot be $\tcpa$-constrained since their cost for any impression they are winning cannot be more than their bid $b_{j,i} = \alpha_j(\r) v_{j,i} < T_j v_{j,i}$. Thus, their $\tcpa$ constraint, i.e., the first constraint in Problem~\eqref{con:x}, is not tight, and hence, by increasing their bidding parameter to $T_j$, the bidder can only increase the total value without violating its $\tcpa$ constraint. In summary, we make the following assumption:

\begin{assumption}[Uniform Undominated Bidding]\label{lem:tcpa-bid-atleast-tcpa}
Each bidder $j\in J$ uses uniform bidding, i.e., $\forall i\in I,\,b_{j,i}(\r) = \alpha_j(\r) v_{j,i}$ for some bidding parameter $\alpha_j(\r)\ge 0$. Moreover, each $\ql$ bidder $j$ uses a bidding parameter $\alpha_j(\r) = 1$, and each $\tcpa$ bidder $j$ uses a bidding parameter $\alpha_j(\r)\geq T_j$.
\end{assumption}

The equilibrium solution we adopt for the bidders' subgame is a version of subgame perfection that takes into account endogenous tie-breaking rules, which is in line with the literature, e.g., the pacing equilibrium for $\budgeted$ bidders~\citep{conitzer2021multiplicative} and the autobidding equilibrium for $\tcpa$ bidders~\citep{li2022auto}.

\begin{definition}[Subgame Bidding Equilibrium]\label{def:uniform_bidding_equilibrium}
Consider the bidders' subgame given reserve prices $\r$ posted by the channels. An equilibrium for the subgame consists of bidders' bidding parameters $\boldsymbol{\alpha}(\r) = (\alpha_j(\r))_{j\in J}$ and probabilities of allocations of the impressions $\x(\r) = (x_{j,i}(\r))_{j \in J,i\in I}$ such that
\begin{enumerate}
    \item[(1)] Only a bidder whose bid is no less than the cost gets the impression: for $i\in I_k$, $x_{j,i}(\r)>0$ holds only if $b_{j,i}(\r)\ge c_{j,i}(\b_i(\r),\r)$.
    \item[(2)] Full allocation of any item with a bid above the reserve price: for $i\in I_k$, $\sum_{j\in J} x_{j,i}(\r)=1$ must hold if there exists some $\ell\in J$ such that $b_{\ell,i}(\r)> r_{\ell,i}$.
    \item[(3)] Constraints are satisfied: for each $j\in J_{\tiny \budgeted}$, $\sum_{i\in I}c_{j,i}(\b_i(r),\r)\cdot x_{j,i}(\r)\le B_j$, and for each $j\in J_{\tiny \tcpa}$, ${\sum_{i\in I}c_{j,i}(\b_i(\r),\r) x_{j,i}(\r)} \le T_j \cdot {\sum_{i\in I}v_{j,i}x_{j,i}(\r)}$.
    \item[(4)] For every Budgeted or tCPA bidder $j$, even if they can decide the fraction $x_{j,i}(\r)$ of an impression $i$ they get in case they are tied for impression $i$, increasing their bidding parameter would not increase their value without violating their budget/tCPA constraint.
\end{enumerate}
\end{definition}

The existence of subgame bidding equilibrium is a straightforward consequence by adapting the existence proofs of the pacing equilibrium for $\budgeted$ bidders~\citep{conitzer2021multiplicative} and the autobidding equilibrium for $\tcpa$ bidders~\citep{li2022auto}.
\begin{proposition}\label{prop:subgame_equilibrium_exists}
In the bidders' subgame, the subgame bidding equilibrium always exists.
\end{proposition}

\begin{comment}% DO NOT remove -- useful if we write our own proof instead of citing their results
The next fact will help us prove the existence of uniform-bidding equilibrium.

\begin{fact}\label{fact:cap}
Given a second-price uniform-bidding game, let $T_{max}=\max_{j\in J_{\tiny \tcpa}} T_j$, $B_{max}=\max_{j\in J_{\tiny \budgeted}} B_j$, $v_{min}=\min_{j\in J, i\in I \textnormal{ s.t. } v_{j,i}>0} v_{j,i}$, $v_{max}=\max_{j\in J, i\in I \textnormal{ s.t. } v_{j,i}>0} v_{j,i}$, $v_{sum}=\sum_{j\in J, i\in I} v_{j,i}$, $p_{max}=\max_{i\in I} p_i$, $r_{max}=\max_{k\in K} r_k$, and let $U>\max\{\frac{|J|\cdot T_{max}\cdot v_{sum}}{v_{min}},\, \frac{|J|\cdot B_{max}}{v_{min}},\, \frac{|J|v_{max}}{v_{min}},\, p_{max},\, r_{max}\}$. For any $(\boldsymbol{\alpha}, \mathbf{x})$ that satisfies the first three items of Definition~\ref{def:uniform_bidding_game}, we have that
\begin{itemize}
    \item if a bidder $j\in J$ has a bidding parameter $\alpha_j\ge U$, they will win all the impressions with non-zero value to them, i.e., for all $i\in I$ such that $v_{j,i}>0$, we have $x_{j,i}=1$.
    %\item Moreover, if we let $\alpha_j=U$ instead, the bidder $j$ still wins all the impressions with non-zero value, and $(\boldsymbol{\alpha}, \mathbf{x})$ is still a uniform-bidding equilibrium.
\end{itemize}
\end{fact}
\begin{proof}
Suppose for contradiction that there is a bidder $j^*\in J$ who has a bidding parameter $\alpha_{j^*}\ge U$ but does not fully win certain impression $i^*\in I_{k^*}$ such that $v_{j^*,i^*}>0$ (i.e., $x_{j^*,i^*}<1$).
We first show that $U\cdot v_{j^*,i^*} >r_{j^*,i^*}$, which implies $b_{j^*,i^*}>r_{j^*,i^*}$ because $b_{j^*,i^*}=\alpha_{j^*}v_{j^*,i^*}$ and $\alpha_{j^*}\ge U$. Specifically, by our assumption,
$U>\max\{r_{max},\,p_{max}\}$, and thus, $U\cdot v_{j^*,i^*}> \max\{r_{max},\,p_{max}\}v_{j^*,i^*}\ge \max\{r_{k^*},\,p_{i^*}\}v_{j^*,i^*}=r_{j^*,i^*}$.

Then, it follows from $b_{j^*,i^*}>r_{j^*,i^*}$ and item (1) of Definition~\ref{def:uniform_bidding_equilibrium} that the price for impression $i^*$ is at least $b_{j^*,i^*}\ge U\cdot v_{j^*,i^*}$. Moreover, by $b_{j^*,i^*}>r_{j^*,i^*}$ and item (2) of Definition~\ref{def:uniform_bidding_equilibrium}, we have that $\sum_{j\in J}x_{j,i^*}=1$, and it follows that there must be a bidder $\ell\in J$ such that $x_{\ell,i^*}\ge 1/|J|$, which implies that the bidder $\ell$ pays at least $U\cdot v_{j^*,i^*}/|J|$.
Furthermore, we derive that
\begin{align*}
    \frac{U\cdot v_{j^*,i^*}}{|J|}&>\max\{\frac{|J|\cdot T_{max}\cdot v_{sum}}{v_{min}},\, \frac{|J|\cdot B_{max}}{v_{min}},\, \frac{|J|v_{max}}{v_{min}}\}\cdot \frac{v_{j^*,i^*}}{|J|} &&\text{(By our assumption for $U$)} \\
    &=\max\{T_{max}\cdot v_{sum}\cdot\frac{v_{j^*,i^*}}{v_{min}},\, B_{max}\cdot\frac{v_{j^*,i^*}}{v_{min}},\, v_{max}\cdot\frac{v_{j^*,i^*}}{v_{min}}\} \\
    &\ge\max\{T_{max}\cdot v_{sum},\, B_{max},\, v_{max}\} &&\text{(By definition of $v_{min}$)}.
\end{align*}
Hence, the cost of impression $i^*$ to the bidder $\ell$ is strictly larger than $\max\{T_{max}\cdot v_{sum},\, B_{max}, v_{max}\}$. Notice that $\ell$ cannot be a QL bidder because otherwise $\ell$ bids at most $v_{\ell,i^*}\le v_{max}$ for impression $i^*$, and by item (1) of Definition~\ref{def:uniform_bidding_equilibrium}, $\ell$ should not have won any fraction of $i^*$ in the equilibrium. Moreover, if $\ell\in J_{\tiny \budgeted}$, then $\ell$'s budget constraint is violated because $\ell$'s payment is strictly larger than $B_{max}\ge B_{\ell}$, and if $\ell\in J_{\tiny \tcpa}$, then $\ell$'s tCPA constraint is violated because $\ell$'s total utility is at most $\sum_{i\in I}v_{j,i}$, and thus $\ell$'s payment per utility is strictly larger than $\frac{T_{max}\cdot v_{sum}}{\sum_{i\in I}v_{j,i}}\ge T_{max}\ge T_{\ell}$. Either case contradicts item (3) of Definition~\ref{def:uniform_bidding_equilibrium}.
\end{proof}
\end{comment}

\subsection{Channels}

We focus on two models that depend on the objective functions the channels may have: the {\em Local} channels model and the {\em Global} channels model.

{\bf Local Channels Model}: In this case, each channel sets its reserve price $r_k$ to maximize its own revenue given the other channels' reserve prices $\r_{-k}$. Thus, channel $k$ solves
$$ \max_{r_k} \sum_{j\in J}\sum_{i \in I_k} c_{j,i}(\b_i(r_k, \r_{-k}),r_k,\r_{-k})x_{j,i}(r_k,\r_{-k}).$$
\medskip

{\bf Global Channels Model}: In this case, the channels determine the reserve prices $\r$ to maximize the sum of the revenue across all channels. Thus, they set reserve prices solving
$$ \max_{\r} \sum_{k\in K} \sum_{j\in J}\sum_{i \in I_k} c_{j,i}(\b_i(\r),\r)x_{j,i}(\r).$$

%\begin{remark}
%A generalized version from the previous two models considers a partition of the set of channels and assumes that channels belonging to the same partition would set their reserve prices to maximize the sum of the partition's revenue. This general model is beyond the scope of this paper.\Junyao{Move this to future directions?}\Andres{Agree}
%\end{remark}

\subsection{The Full Game}
We summarize the full game for the channels and the bidders as the following two-stage game:
\begin{itemize}
    \item[(S0)] Each Channel $k\in K$ chooses a uniform reserve price (in the cost-per-unit-value space) $r_k$ with finite precision\footnote{Note that assuming the reserve prices have finite precision is very natural for practice.} for their impressions $I_k$.
    \item[(S1)] Each Bidder $j\in J$ observes the reserve prices $\r$ posted by the channels (and the reserve prices $(p_i)_{i\in I}$ prechosen by the publishers), and then they choose a bidding parameter $\alpha_j(\r)$ and submit their bids according to $\alpha_j(\r)$ (see Assumption~\ref{lem:tcpa-bid-atleast-tcpa}). If Bidder $j$ is tied for impression $i$, they can also decide the fraction $x_{j,i}(\r)$ of impression $i$ they get.
\end{itemize}

By Proposition~\ref{prop:subgame_equilibrium_exists}, given any fixed $\r$ in the support of the channels' mixed strategies, stage (S1) has a subgame equilibrium between the bidders. We assume that stage (S1) always results into one such equilibrium deterministically, i.e., henceforth, we assume that $((\b_i(\r))_{i\in I},\x(\r))$ in stage (S1) is always a fixed subgame equilibrium given $\r$ (as defined in Definition~\ref{def:uniform_bidding_equilibrium}).

Channels are allowed to use mixed strategies in stage (S0), i.e., sampling their reserve price $r_k$ from a distribution $\mathcal{R}_k$. Notice that the game for the channels is a finite game between finite players, and hence, there always exists a mixed-strategy equilibrium by the celebrated Nash's theorem~\cite{nas1951non}.
%\ganote{add the citation to non-cooperative games}

Additionally, we assume the game is complete-information. That is,  $(v_{j,i}, B_j, T_j, p_i)_{j\in J, i\in I}$ are known to the channels and the bidders.
%\Junyao{In the intro, we need to provide ample motivation for this assumption as well as why channels can set reserve prices in cost-per-unit-value space.}\Andres{We can claim that this is the 1st paper studying this and we start with basic setup of complete info as in \cite{AggarwalBM19}. Is this enough? Regarding the cost-per-unit-value space, I agree we need to motivate it well. If $v_{j,i}$ are pctrs then we are charging only if there is click. Also, we can extend to reserve price in the dollar space by suffering a $log(v_max/v_min)$ right?}

\subsection{Important Concepts}
We now present the main concepts which we will use to compare the outcomes of the local channels model to the global channels model.

\begin{definition}[Liquid Welfare]\label{def:liquid_wel}
The liquid welfare of a fractional allocation $\x =(x_{j,i})_{j\in J, i \in I}$ is
$$ {Wel}(\x) =  \sum_{j\in J_{\tiny \budgeted}}\min\left\{ \budget_j, \sum_{i\in I} v_{j,i} x_{j,i} \right\}+ \sum_{j \in J_{\tiny \tcpa }} \sum_{i\in I} T_jv_{j,i} x_{j,i} + \sum_{j \in J_{\tiny \ql }} \sum_{i\in I} v_{j,i} x_{j,i},$$
and the optimal liquid welfare is
$Wel^*:= \max_{\x \textrm{ that satisfies bidders' constraints}} Wel(\x)$.
\end{definition}

This concept of liquid welfare has been previously studied in e.g., \citet{AggarwalBM19} and \citet{azar2017liquid}, and it was first introduced by \citet{dobzinski2014efficiency}. It is well-known that optimal liquid welfare is an upper bound on the sum of the revenues of all channels. More precisely, optimal liquid welfare $Wel^*$ is greater or equal than the sum of the channels' revenues, which we denote by $Rev(\r):=\sum_{k\in K} \sum_{j\in J}\sum_{i \in I_k} c_{j,i}(\b_i(\r),\r)x_{j,i}(\r)$, regardless of the reserve prices they choose:

\begin{fact}
\label{fact:rev-wel}
For any $\r\in\R_{\ge0}^K$, $Rev(\r) \leq Wel^*$.
\end{fact}

Thus, we use the optimal liquid welfare as the benchmark to measure performance of the revenue in the local and global models. We let $\mbox{LocalEQ}$ denote the set that contains every mixed-strategy equilibrium $\mathcal{R}:=(\mathcal{R}_k)_{k\in K}$ for the channels in the local channel model, and we define the revenue guarantees in the local and global models as follows:

\begin{definition}[Revenue Guarantee]\label{def:rev_guarantee}
The revenue guarantees for the local and global models are defined as 
\begin{align*} 
RevG(Local) &= \frac{\inf_{\mathcal{R}\in \mbox{LocalEQ}} \E_{\r\sim\mathcal{R}}[\mbox{Rev}(\r)]}{Wel^*},\\
 RevG(Global) &= \frac{\sup_{\r\in\R_{\ge0}^K} \mbox{ Rev}(\r)}{Wel^*}.
\end{align*}
\end{definition}

Note that any reserve prices $\r$ in the support of any $\mathcal{R}\in\mbox{LocalEQ}$ in the local model is also feasible in the global model, thereby giving us the following fact.
\begin{fact}
\label{fact:local-global}
$RevG(Local) \leq RevG(Global) \leq 1$
\end{fact}

\medskip

Furthermore, to compare the outcomes of the two models, we use the standard notion of the Price of Anarchy~\cite{koutsoupias-poa}. 
\begin{definition}[Price of Anarchy]\label{def:poa}
The Price of Anarchy (PoA) of the local model compared to the global model is
$$\mbox{PoA} \;=\; \frac{\inf_{\mathcal{R}\in \mbox{LocalEQ}} \E_{\r\sim\mathcal{R}}[\mbox{Rev}(\r)]}{ \sup_{\r\in\R_{\ge0}^K} \mbox{ Rev}(\r)}.$$
\end{definition}

==> multi_channel (1)/03-hardness.tex <==
\section{Hardness of equilibrium computation}
\label{sec:hardness}
In this section, we study the computational complexity of computing equilibrium of our game. Our main result in this section is that we show that even just finding the subgame equilibrium (Definition~\ref{def:uniform_bidding_equilibrium}) for the bidders' subgame is already computationally hard:
\begin{theorem}
\label{thm:subgame-hardness}
Finding the subgame equilibrium (Definition~\ref{def:uniform_bidding_equilibrium}) is $\PPAD$-hard.
\end{theorem}

We prove this by reduction from the problem of finding an approximate Nash equilibrium for the 0-1 bimatrix game, which was shown to be $\PPAD$-hard in~\cite{CTV07}. The  basic  idea  of the proof is similar to that of the hardness result for finding a pacing equilibrium for budget-constrained quasi-linear bidders~\cite{CKK21}. However, we have to handle many difficulties that are unique to $\tcpa$ bidders.  Most notably, in contrast to budget-constrained quasi-linear bidders, whose bidding parameters are at most $1$, $\tcpa$ bidders do not have a natural upper bound for their bids, and their bidding parameters can be arbitrarily high when their $\tcpa$ constraints are not tight. We construct new gadgets that force $\tcpa$ bidders' bidding parameters to stay bounded but still leave a controlled amount of "slack" for them, so that they can bid on impressions that are more expensive than their $\tcpa$ but not win all of them. We provide the full reduction in the appendix.

Despite the computational hardness, we are able to prove tight revenue guarantees that channels can achieve in the equilibrium, which we will present in the subsequent sections.

==> multi_channel (1)/04-no-pub-prices.tex <==
\section{Revenue and Price of Anarchy with no Publisher Reserves}\label{zero-publisher-reserve}
In this section, we focus on the setting where impressions do not have publisher-chosen reserve prices, i.e. $p_i =0$ for every $i\in I$. We study the revenue guarantees that the channels can achieve in the local model where each channel chooses their reserve price out of their own self-interest vs. the global model where the channels cooperatively choose the reserve prices to maximize their total revenue. 

Our main results in this section are the following:
%\ganote{update these as per intro. Also need 1/log-ratio which is not nice. maybe just say that revenus is a blah fraction or welfare is no more than .. or gap is...}
\begin{itemize}
    \item We establish a revenue guarantee (defined in Definition~\ref{def:rev_guarantee}) in the local model (Theorem~\ref{thm:rev-local}).
    \item Moreover, we prove that our revenue guarantee in the local model is \emph{tight even for the global model} (Proposition~\ref{ex:revg-ub}).
    \item Furthermore, as a corollary of the revenue guarantee in the local model, we immediately get a lower bound for the price of anarchy (Theorem~\ref{lem:ineq-POA}). We give a matching upper bound for the price of anarchy (Theorem~\ref{lem:tight-PoA}) and thus establish a \emph{tight separation between the local and global models}.
\end{itemize}

\subsection{Revenue Guarantees}

We begin by proving the main technical result of this section, which establishes a revenue guarantee for the local model. 
It is $\PPAD$-hard to actually compute the equilibrium, as shown in Theorem~\ref{thm:subgame-hardness}. Nevertheless, we will show that each channel can set a certain reserve price in order to guarantee itself a decent amount of revenue, irrespective of the reserve prices set by other channels.

To do this, we will show that each channel can set a reserve price which ensures that its revenue is at least a certain fraction of the total budget of
%contribution to OLW is hard to define for budgeted. changing.
%its contribution to the optimal liquid welfare (Definition~\ref{def:liquid_wel}) 
unconstrained $\budgeted$ bidders (Lemma~\ref{lem:budgeted-uniform} and Corollary~\ref{cor:min-rev-budg}). Then, we will show that each channel can set a reserve price which ensures that its revenue is at least a certain fraction of its contribution to the optimal liquid welfare (Definition~\ref{def:liquid_wel}) from $\tcpa$ and $\ql$ bidders (Lemma~\ref{lem:tcpa-ql} and Corollary~\ref{cor:tcpa-ql-rev}).
Finally, we will put these together to get the final revenue guarantee (Theorem~\ref{thm:rev-local}).

The main difficulty in this proof comes from $\budgeted$ bidders who are unconstrained, i.e. not spending their budget, at the equilibrium of the local model. The contribution to optimal Liquid Welfare from $\tcpa$ and $\ql$ bidders can be easily attributed to different channels (see the definition of $W_{\tiny \tcpa}^*(k)$ and $W_{\tiny \ql}^*(k)$ in \ref{lem:tcpa-ql}) and there is a natural way for a channel to obtain a good fraction of its contribution as revenue (see Lemma~\ref{lem:tcpa-ql}). However, there is no obvious attribution for the contribution of $\budgeted$ bidders to different channels, and no obvious lower bound on the bid of $\budgeted$ bidders. In order to get a handle on unconstrained $\budgeted$ bidders, we define the notion of {\em Budget-fraction}. 
%The key notion that will be helpful for lower bounding the revenue from $\budgeted$ bidders is a ratio that we call the budget-fraction:
\begin{definition}[Budget-fraction $\beta_j$ and $\beta_{max}$, $\beta_{min}$]\label{def:budget-fraction}
For a $\budgeted$ bidder $j$, define their budget-fraction as $\beta_j = \frac{B_j}{\sum_{i\in I} v_{j,i}}$, i.e., the ratio of their budget to the sum of their values of all impressions.
Also, define $\beta_{max} = \max_{j \in J_{\tiny \budgeted}} \beta_j$ and $\beta_{min} = \min_{j \in J_{\tiny \budgeted}} \beta_j$.
\end{definition}
Intuitively, the budget-fraction for a $\budgeted$ bidder plays a role similar to the $\tcpa$ of a $\tcpa$ bidder. With this, we are ready to prove some key technical claims that will help establish a lower bound on the bids of unconstrained $\budgeted$ bidders, which in turn will help us find a good reserve price for these bidders.

\subsection*{Key Claims} 
\begin{claim}
\label{lem:unconstrained-win-all}
In a subgame equilibrium (Definition~\ref{def:uniform_bidding_equilibrium}), if a $\budgeted$ bidder $j$ is unconstrained, i.e. not spending all its budget, then they must be winning all impressions $i$ with $v_{j,i} > 0$ and cannot be tied with another unconstrained $\budgeted$ bidder on those impressions.
\end{claim}
\begin{proof}
Suppose for contradiction that a $\budgeted$ bidder $j$ is unconstrained but does not fully win certain impression $i$ (i.e., $x_{j,i}(\r)<1$) such that $v_{j,i}>0$. Notice that Bidder $j$ can increase the bidding parameter $\alpha_j$ without increasing the total spend until Bidder $j$ is tied for (but does not fully win) some impression $i'$ with $v_{j,i'}>0$. Such tie must occur, because otherwise, as Bidder $j$ increases $\alpha_j$, at some point Bidder $j$ will be tied for the impression $i$. However, this contradicts item (4) of Definition~\ref{def:uniform_bidding_equilibrium}, because Bidder $j$ can strictly increase the utility by increasing $x_{j,i'}(\r)$ by a sufficiently small amount such that their budget constraint is not violated.
\end{proof}
The next claim follows directly from Claim~\ref{lem:unconstrained-win-all}.
\begin{claim}
\label{cor:one-unbudgeted}
In a subgame equilibrium, for any impression $i\in I$, there can be at most one unconstrained $\budgeted$ bidder $j$ with $v_{j,i} > 0$.
\end{claim}

Next we prove the following claim, which will be helpful in bounding revenue against the optimal Liquid Welfare from unconstrained $\budgeted$ bidders. 
%The following claim helps establish a connection between a lower for $\budgeted$ bidders.
\begin{claim}
\label{lem:bid-atleast-budget-fraction}
If the final reserve price of an impression $i$ for a $\budgeted$ bidder $j$ satisfies that $r_{j,i}<\beta_j v_{j,i}$, then impression $i$ will be sold for a cost at least $r_{j,i}$ in the subgame equilibrium.
\end{claim}
\begin{proof}
We first show that unless impression $i$ is fully sold to bidder $j$ (in which case the statement holds trivially because the cost of impression $i$ is at least its reserve price $r_{j,i}$), Bidder $j$ will bid $b_{j,i} \geq \beta_j v_{j,i}$ for impression $i$.

Suppose $b_{j,i} < \beta_j v_{j,i}$ for contradiction. Recall that $\alpha_j$ denotes the bidding parameter of Bidder $j$. Since $b_{j,i} = \alpha_j v_{j,i}$ is assumed to be less than $\beta_j v_{j,i}$, we get $\alpha_j < \beta_j$.
Moreover, because the total amount spent by Bidder $j$ is at most the sum of their bids, we have that $$\mbox{Total amount spent by bidder } j \leq \sum_{i\in I} b_{j,i} = \sum_{i\in I} \alpha_j v_{j,i} < \sum_{i\in I} \beta_j v_{j,i} = B_j.$$
Thus, Bidder $j$ is unconstrained. By Claim~\ref{lem:unconstrained-win-all}, this bidder must be winning all its impressions.

Now we have shown that $b_{j,i}\ge\beta_j v_{j,i}$, which is by our assumption strictly greater than $r_{j,i}$. Thus, it follows from item (2) of Definition~\ref{def:uniform_bidding_equilibrium} that impression $i$ will be fully sold in the subgame equilibrium (for a cost that is at least $b_{j,i}>r_{j,i}$ because of item (1) of Definition~\ref{def:uniform_bidding_equilibrium}).
\end{proof}

The following claim, analogous to the claim above, will be used to bound revenue against the optimal Liquid Welfare from $\tcpa$ and $\ql$ bidders.
\begin{claim}
\label{lem:sold-at-rji}
If the final reserve price (i.e., in the cost space) of impression $i$ for a $\tcpa$ bidder $j$ (recall this is denoted by $r_{j,i}$ in the model section) satisfies that $r_{j,i}<T_j v_{j,i}$, then impression $i$ will be sold for a cost of at least $r_{j,i}$ in the subgame equilibrium. Similarly, if the final reserve price of impression $i$ for a $\ql$ bidder $j$ satisfies that $r_{j,i}<v_{j,i}$, then impression $i$ will be sold for a cost of at least $r_{j,i}$ in the subgame equilibrium.
\end{claim}
\begin{proof}
By Assumption~\ref{lem:tcpa-bid-atleast-tcpa}, a $\tcpa$ bidder $j$ bids $b_{j,i}(\r) \geq T_j v_{j,i}>r_{j,i}$ on impression $i$. Thus, by item (2) of Definition~\ref{def:uniform_bidding_equilibrium}, impression $i$ will be fully sold in the subgame equilibrium (for a cost that is at least $r_{j,i}$ because of item (1) of Definition~\ref{def:uniform_bidding_equilibrium}). An analogous argument holds for the case of $\ql$ bidder.
\end{proof}

Next, we first lower bound each channel's revenue against the optimal Liquid Welfare contribution from $\budgeted$ bidders (Lemma~\ref{lem:budgeted-uniform} and Corollary~\ref{cor:min-rev-budg}), and then we lower bound each channel's revenue against the welfare contribution from $\tcpa$ and $\ql$ bidders (Lemma~\ref{lem:tcpa-ql} and Corollary~\ref{cor:tcpa-ql-rev}). Finally, we will put these together to get a lower bound on the revenue guarantee (Theorem~\ref{thm:rev-local}). 
%\Junyao{Here is a good place to comment on techniques -- what is standard, what requires some new idea}

\subsection*{Welfare from $\budgeted$ Bidders}
\begin{lemma}
\label{lem:budgeted-uniform}
Let $E$ be any subgame equilibrium given any reserve prices. Define the following:
\begin{itemize}
    \item Let $J^E_C$ be the subset of $\budgeted$ bidders who are {\bf constrained}, i.e. are spending their entire budget in the equilibrium $E$.
    \item Let $J^E_U$ be the subset of $\budgeted$ bidders who are {\bf unconstrained}, i.e. are spending strictly less than their budget in the equilibrium $E$.
    \item For Channel $k$ and $\budgeted$ bidder $j$, let $\rho(k,j) = \frac{\sum_{i \in I_k} v_{j,i}}{\sum_{i\in I} v_{j,i}}$ be the ratio of the total value of impressions in $I_k$ for Bidder $j$ to the total value of all impressions in $I$ for Bidder $j$.
\end{itemize}
Then, for any $\varepsilon>0$,
\begin{enumerate}
    \item in the equilibrium $E$, the total revenue of all the channels from a Bidder $j \in J^E_C$ is no less than their budget $B_j$,
    \item and moreover, if Channel $k$ could set bidder-specific reserve prices $r_k(j) = (1-\varepsilon)\beta_j$ for each $\budgeted$ bidder $j$ (recall $\beta_j$ is the budget-fraction in Definition~\ref{def:budget-fraction}), then regardless of other channels' reserve prices, in the resulting subgame equilibrium (this is not necessarily $E$), Channel $k$ can obtain a revenue of at least $$\sum_{j \in J^E_U} (1-\varepsilon)\rho(k,j) B_j,$$
    \item and furthermore, Channel $k$ can set a uniform reserve price $r_k$ which is independent of $E$ such that regardless of other channels' reserve prices, in the resulting subgame equilibrium (not necessarily $E$), Channel $k$ will obtain a revenue of at least
    $$\frac{\sum_{j \in J^E_U} (1-\varepsilon)\rho(k,j) B_j} {2\max \big\{1,\big\lceil \log \frac{\beta_{max}}{\beta_{min}}\big\rceil\big\}}.$$
\end{enumerate}
\end{lemma}

\begin{proof}
\begin{enumerate}
\item Since bidders $j \in J^E_C$ are spending their entire budget in $E$ (by definition of $J^E_C$), the total revenue of all channels from them is equal to their budget.

\item Consider any equilibrium $E_r$ resulting from Channel $k$'s bidder-specific reserve prices given in the statement and arbitrary reserve prices of other channels (note $E_r$ is unrelated to $E$). Consider any impression $i \in I_k$. Since Channel $k$ has set a bidder-specific reserve price of $(1-\varepsilon)\beta_j$ for each $\budgeted$ bidder $j$, the reserve price of impression $i$ for $\budgeted$ bidder $j$ is $r_{j,i} =(1-\varepsilon)\beta_j v_{j,i}<\beta_j v_{j,i}$. Then, by Claim~\ref{lem:bid-atleast-budget-fraction}, each impression $i$ is sold for a price of at least $r_{j,i} = (1-\varepsilon)\beta_j v_{j,i}$ in the equilibrium $E_r$ for any $j\in J_{\tiny \budgeted}$. That is,
\begin{equation}\label{eq:revk_budget_frac}
    \textrm{the revenue of Channel $k$ in the equilibrium $E_r$} \geq \sum_{i \in I_k} \max_{j \in J_{\tiny \budgeted}} (1-\varepsilon)\beta_j v_{j,i}.
\end{equation}

Now let $I_k(j) \subseteq I_k$ denote the set of the impressions $i\in I_k$ such that $v_{j,i} > 0$. By Claim~\ref{cor:one-unbudgeted}, if $j$ and $j'$ are two bidders unconstrained in the equilibrium $E$, then $I_k(j)$ and $I_k(j')$ are disjoint.

Hence, we have that
\begin{align}
    \sum_{i \in I_k} \max_{j \in J_{\tiny \budgeted}} (1-\varepsilon)\beta_j v_{j,i}
    & \geq \sum_{j \in J^E_U} \sum_{i \in I_k(j)} (1-\varepsilon)\beta_j v_{j,i}  \label{eq:budg1_first}\\
    & = \sum_{j \in J^E_U} (1-\varepsilon)\beta_j \sum_{i \in I_k(j)} v_{j,i} \\
    & = \sum_{j \in J^E_U} (1-\varepsilon)\beta_j \rho(k,j) \sum_{i\in I} v_{j,i} \\
    & = \sum_{j \in J^E_U} (1-\varepsilon)\rho(k,j) B_j \label{eq:budg1_last},
\end{align}
which finishes the proof by Inequality~\eqref{eq:revk_budget_frac}.

\item The high-level idea for setting a good uniform reserve price is to bucketize the reserve prices and pick the one with the highest revenue potential. Specifically, we divide $\budgeted$ bidders into the following buckets:
$$J^s_{\tiny \budgeted} = \{j: j \in J_{\tiny \budgeted} \mbox{ and } 2^s \beta_{min} \leq \beta_j \leq 2^{s+1} \beta_{min}\}$$
for $s\in\{0\}\cup\left[\lceil \log \frac{\beta_{max}}{\beta_{min}} \rceil-1\right]$ (recall $\beta_{max},\beta_{min}$ are the largest and smallest budget-fractions respectively defined in Definition~\ref{def:budget-fraction}).
We observe that if Channel $k$ sets its uniform reserve price to $(1-\varepsilon)2^{s} \beta_{min}$, then for bidders $j \in J^s_{\tiny \budgeted}$, it holds that $r_{j,i}=(1-\varepsilon)2^{s} \beta_{min}v_{j,i}<\beta_j v_{j,i}$ for all impressions $i\in I_k$. Thus, by Claim~\ref{lem:bid-atleast-budget-fraction}, each impression $i\in I_k$ will get sold for a price of at least $\max_{j \in J^s_{\tiny \budgeted}} r_{j,i}=\max_{j \in J^s_{\tiny \budgeted}} (1-\varepsilon)2^{s} \beta_{min}v_{j,i} \geq \max_{j \in J^s_{\tiny \budgeted}} \frac{1-\varepsilon}{2} \beta_j v_{j,i}$ (the inequality is by bucketization) in the subgame equilibrium $E_r$ that results from Channel $k$ setting a uniform reserve price of $(1-\varepsilon)2^{s} \beta_{min}$ and arbitrary reserve prices set by other channels. Thus, the revenue of Channel $k$ from setting a uniform reserve price to $(1-\varepsilon)2^{s} \beta_{min}$
\begin{align}\label{eq:revk_per_bucket}
\mbox{Rev}_k((1-\varepsilon)2^{s} \beta_{min}) 
& \geq \sum_{i \in I_k} \max_{j \in J^s_{\tiny \budgeted}} \frac{1-\varepsilon}{2} \beta_j v_{j,i}.
\end{align}

Now let $I_k(j) \subseteq I_k$ denote the set of impressions $i\in I_k$ such that $v_{j,i} > 0$. Then, by Claim~\ref{cor:one-unbudgeted}, $I_k(j)$ and $I_k(j')$ are disjoint for two unconstrained $\budgeted$ bidders $j\neq j'$ in the equilibrium $E$. Hence, we have that
\begin{align}\label{eq:revk_sum_over_buckets}
    \sum_s \sum_{i \in I_k} \max_{j \in J^s_{\tiny \budgeted}} \frac{1-\varepsilon}{2} \beta_j v_{j,i}&\ge \sum_s \sum_{j \in J^E_U\cap J^s_{\tiny \budgeted}}\sum_{i \in I_k(j)} \frac{1-\varepsilon}{2} \beta_j v_{j,i}\nonumber\\
    &=\sum_{j \in J^E_U}\sum_{i \in I_k(j)} \frac{1-\varepsilon}{2} \beta_j v_{j,i}\nonumber\\
    &\ge\frac{1-\varepsilon}{2} \sum_{j \in J^E_U} \rho(k,j) B_j,
\end{align}
where the last inequality follows from the same derivation as in Inequalities~(\ref{eq:budg1_first}-\ref{eq:budg1_last}).

Finally, let $s^*=\argmax_{s\in\{0\}\cup\left[\lceil \log \frac{\beta_{max}}{\beta_{min}} \rceil-1\right]}\sum_{i\in I_k}\max_{j \in J^s_{\tiny \budgeted}} \frac{1-\varepsilon}{2} \beta_j v_{j,i}$. Then, we have that the revenue of Channel $k$ by setting a uniform reserve price $r_k^* = 2^{s^*} \beta_{min}$ (notice $r_k^*$ is indeed independent of $E$) is
\begin{align*}
\mbox{Rev}_k((1-\varepsilon)2^{s^*} \beta_{min}) 
& \geq \sum_{i \in I_k} \max_{j \in J^s_{\tiny \budgeted}} \frac{1-\varepsilon}{2} \beta_j v_{j,i} &&\text{(By Inequality~\eqref{eq:revk_per_bucket})}\\
&\ge \frac{\sum_s \sum_{i \in I_k} \max_{j \in J^s_{\tiny \budgeted}} \frac{1-\varepsilon}{2} \beta_j v_{j,i}}{\max\big \{1, \big \lceil \log \frac{\beta_{max}}{\beta_{min}}\big \rceil \big \}} &&\text{(By definition of $s^*$)}\\
&\ge \frac{\frac{1-\varepsilon}{2} \sum_{j \in J^E_U} \rho(k,j) B_j}{\max\big \{1, \big \lceil \log \frac{\beta_{max}}{\beta_{min}}\big \rceil \big \}} &&\text{(By Inequality~\eqref{eq:revk_sum_over_buckets})}.
\end{align*}
\end{enumerate}
\end{proof}

%Similar to Corollary~\ref{cor:tcpa-ql-rev}, 
Item (3) in Lemma~\ref{lem:budgeted-uniform} implies the following corollary:
\begin{corollary}
\label{cor:min-rev-budg}
Define $\rho(k,j)$ as in Lemma~\ref{lem:budgeted-uniform}. Let $\mathcal{R}=(\mathcal{R}_k)_{k\in K}$ be any mixed-strategy equilibrium of the channels' game (i.e., S0), and let $E(\r)$ be the subgame equilibrium given any reserve prices $\r$ in the support of the channels' mixed strategies. Then, the expected revenue of Channel $k$ in the mixed-strategy equilibrium $\mathcal{R}$ is at least 
$$\mathbf{E}_{\r\sim \mathcal{R}}\left[\frac{\sum_{j \in J^{E(\r)}_U} (1-\varepsilon)\rho(k,j) \budget_j}{2\max\big \{1, \big \lceil \log \frac{\beta_{max}}{\beta_{min}}\big \rceil \big \}}\right].
$$
\end{corollary}

\subsection*{Welfare from $\tcpa$ and $\ql$ Bidders}
\begin{lemma}
\label{lem:tcpa-ql}
Let $\x^*$ be a welfare maximizing allocation (i.e., $\x^*$ is s.t. $Wel^*=Wel(\x^*)$ in Definition~\ref{def:liquid_wel}) 
and
\begin{itemize}
    \item let $W_{\tiny \tcpa}^*(k)$ be the liquid welfare generated by the impressions in $I_k$ allocated to $\tcpa$ bidders in $x^*$, i.e.,
    $$W_{\tiny \tcpa}^*(k):=\sum_{j \in J_{\tiny \tcpa }} \sum_{i\in I_k} T_jv_{j,i} x^*_{j,i},$$
    \item and let $W_{\tiny \ql}^*(k)$ be the liquid welfare generated by the impressions in $I_k$ allocated to quasi-linear bidders in $x^*$, i.e.,
    $$W_{\tiny \ql}^*(k):=\sum_{j \in J_{\tiny \ql }} \sum_{i\in I_k} v_{j,i} x^*_{j,i}.$$
\end{itemize}

Then, for any $\varepsilon>0$,
\begin{enumerate}
\item if Channel $k$ could set the bidder-specific reserve prices (also in the cost-per-unit-value space) $r_k(j)$ for each $\tcpa$ or $\ql$ bidder $j$ as follows:
\begin{equation*}
r_k(j) = \begin{cases}
(1-\varepsilon)T_j &\text{if $j$ is a $\tcpa$ bidder} \\
1-\varepsilon &\text{if $j$ is a $\ql$ bidder},
\end{cases}
\end{equation*}
then Channel $k$ obtains a revenue at least $(1-\varepsilon)(W_{\tiny \tcpa}^*(k) +W_{\tiny \ql}^*(k))$ regardless of what other channels do,

\item and moreover, we let $T_{max} = \max_{j \in J_{\tiny \tcpa}} T_j$ and let $T_{min} = \min_{j \in J_{\tiny \tcpa}} T_j$, and then Channel $k$ can set a uniform reserve price $r_k$ s.t. Channel $k$ obtains a revenue at least
$$\frac{(1-\varepsilon)(W_{\tiny \tcpa}^*(k) +W_{\tiny \ql}^*(k))}{ 2 + 2\max\big \{1, \big \lceil \log \frac{T_{max}}{T_{min}}\big \rceil \big \}}$$
regardless of what other channels do.
\end{enumerate}
\end{lemma}
\begin{proof}
\begin{enumerate}
    \item  Fix Channel $k$'s bidder-specific reserve prices as in the assumption and consider any subgame equilibrium. For any impression $i \in I_k$, let Bidder $j=\argmax_{\ell\in J_{\tiny \tcpa}\textrm{ s.t. } x^*_{\ell,i}>0} T_{\ell}v_{\ell,i}$, and let Bidder $q=\argmax_{\ell\in J_{\tiny \ql}\textrm{ s.t. } x^*_{\ell,i}>0} v_{\ell,i}$. Since $r_{j,i} =r_k(j)v_{j,i}= (1-\varepsilon)T_j v_{j,i}<T_j v_{j,i}$, it follows from Claim~\ref{lem:sold-at-rji} that impression $i$ will be sold for a cost of at least $r_{j,i}=(1-\varepsilon)T_j v_{j,i}$. Similarly, since $r_{q,i} =r_k(q)v_{q,i}= (1-\varepsilon)v_{q,i}<v_{q,i}$, it follows from Claim~\ref{lem:sold-at-rji} that impression $i$ will be sold for a cost of at least $r_{q,i}=(1-\varepsilon)v_{q,i}$. Moreover, note that the contribution of impression $i$ to $W_{\tiny \tcpa}^*(k)+W_{\tiny \ql}^*(k)$ is at most $\max\{v_{q,i},T_j v_{j,i}\}$, and we have shown impression $i$ will be sold for at least $(1-\varepsilon)$-fraction of this amount, it follows that channel $k$'s revenue is at least $(1-\varepsilon)(W_{\tiny \tcpa}^*(k)+W_{\tiny \ql}^*(k))$.
    
    \item The high-level idea for setting a good uniform reserve price is again to bucketize the bidder-specific reserve prices used above and set the uniform reserve price $r_k$ to the lower end of the bucket that has the highest revenue potential. Specifically, we divide all the $\tcpa$ bidders into the following buckets:
$$J^s_{\tiny \tcpa} = \{j: j \in J_{\tiny \tcpa}, 2^s T_{min} \leq T_j \leq 2^{s+1} T_{min}\}$$
for $s\in\{0\}\cup\left[\lceil \log \frac{T_{max}}{T_{min}} \rceil-1\right]$.

As before, for any impression $i \in I_k$, let bidder $j=\argmax_{\ell\in J_{\tiny \tcpa}\textrm{ s.t. } x^*_{\ell,i}>0} T_{\ell}v_{\ell,i}$ and bidder $q=\argmax_{\ell\in J_{\tiny \ql}\textrm{ s.t. } x^*_{\ell,i}>0} v_{\ell,i}$, and notice that the contribution of impression $i$ to $W_{\tiny \tcpa}^*(k)+W_{\tiny \ql}^*(k)$ is at most $\max\{v_{q,i},T_j v_{j,i}\}$.

If $T_j v_{j,i}>v_{q,i}$, let $s$ be such that $j \in J^s_{\tiny \tcpa}$. Suppose Channel $k$ sets a reserve price of $r_k = (1-\varepsilon)2^s T_{min}$ which is strictly less than $T_j$ because of the bucketization. Then, by Claim~\ref{lem:sold-at-rji}, impression $i$ will be sold at a cost at least $(1-\varepsilon)2^s T_{min} v_{j,i} \geq \frac{1-\varepsilon}{2} T_j v_{j,i}$ in the subgame equilibrium, where the inequality is because of the bucketization.

If $v_{q,i}\ge T_j v_{j,i}$, suppose Channel $k$ sets a reserve price $r_k = 1-\varepsilon$. Then, by Claim~\ref{lem:sold-at-rji}, impression $i$ will be sold at a cost at least $v_{q,i}$ in the subgame equilibrium.

Now we put these two cases together. Let $Rev_k(r_k)$ be the revenue of Channel $k$ at the subgame equilibrium if Channel $k$ sets a uniform reserve price $r_k$ (regardless of the reserve prices of other channels). Then, summing over all the buckets $s$, we have
$$\sum_{r_k\in\{1-\varepsilon,\,T_{min}\}\cup\left\{2^s T_{min}\mid\, s\in\left[\lceil \log \frac{T_{max}}{T_{min}} \rceil-1\right]\right\}} Rev_k(r_k) \geq \frac{1-\varepsilon}{2} (W_{\tiny \tcpa}^*(k)+W_{\tiny \ql}^*(k)),$$
because as we have shown in the above case analysis, all the buckets together cover at least $\frac{1-\varepsilon}{2}$-fraction of the liquid welfare of each impression's contribution to $W_{\tiny \tcpa}^*(k)+W_{\tiny \ql}^*(k)$.

Let $r^*_k = \argmax_{r_k\in\{1-\varepsilon,\,T_{min}\}\cup\left\{2^s T_{min}\mid\, s\in\left[\lceil \log \frac{T_{max}}{T_{min}} \rceil-1\right]\right\}} Rev_k(r_k)$. Then, by setting a reserve price of $r^*_k$, Channel $k$ can get a revenue of at least
$$\frac{(1-\varepsilon)(W_{\tiny \tcpa}^*(k) +W_{\tiny \ql}^*(k))}{ 2 + 2\max\big \{1, \big \lceil \log \frac{T_{max}}{T_{min}}\big \rceil \big \}}.$$
\end{enumerate}
\end{proof}

If Channel $k$ can always get certain amount of revenue by setting a particular uniform reserve price $r_k$ regardless of what other channels do, then Channel $k$'s revenue at any mixed-strategy equilibrium of the channels' game (i.e., stage (S0) of the full game) is at least the same amount (because otherwise Channel $k$ will deviate to the uniform reserve price $r_k$). Thus, item (2) in Lemma~\ref{lem:tcpa-ql} implies the following corollary:
\begin{corollary}
\label{cor:tcpa-ql-rev}
Let $W_{\tiny \tcpa}^*(k)$ and $W_{\tiny \ql}^*(k)$ be defined as in Lemma~\ref{lem:tcpa-ql} above. Then, for any $\varepsilon>0$, at any mixed-strategy equilibrium of the channels' game (S0), the expected revenue of channel $k$ is at least 
$$\frac{(1-\varepsilon)(W_{\tiny \tcpa}^*(k) +W_{\tiny \ql}^*(k))}{ 2 + 2\max\big \{1, \big \lceil \log \frac{T_{max}}{T_{min}}\big \rceil \big \}}.$$
\end{corollary}

\subsection*{The Final Revenue Guarantee}
\begin{theorem} 
\label{thm:rev-local}
For any $\varepsilon>0$,
\begin{equation*}
RevG(Local) \geq \frac{1-\varepsilon}{3 + 2\max\big \{1, \big \lceil \log \frac{T_{max}}{T_{min}}\big \rceil \big \} +2\max\big \{1, \big \lceil \log \frac{\beta_{max}}{\beta_{min}}\big \rceil \big \}}.
\end{equation*}

\end{theorem}
\begin{proof}
Let $\mathcal{R}=(\mathcal{R}_k)_{k\in K}$ be any mixed-strategy equilibrium of the channels' game, and let $E(\r)$ denote the subgame equilibrium given any reserve prices $\r$ in the support of the channels' mixed strategies. Let $\x^*$ be the liquid welfare maximizing allocation (i.e., $\x^*$ is s.t. $Wel^*=Wel(\x^*)$).

By Corollary~\ref{cor:tcpa-ql-rev}, the expected revenue of Channel $k$ in the equilibrium $\mathcal{R}$, denoted by $\mbox{Rev}_k[\mathcal{R}]$, is
$$\mbox{Rev}_k[\mathcal{R}]\ge \frac{(1-\varepsilon)(W_{\tiny \tcpa}^*(k) +W_{\tiny \ql}^*(k))}{ 2 + 2\max\big \{1, \big \lceil \log \frac{T_{max}}{T_{min}}\big \rceil \big \}},$$
where $W_{\tiny \tcpa}^*(k)$ and $W_{\tiny \ql}^*(k)$ are defined as in Lemma~\ref{lem:tcpa-ql}.

Thus, the expected total revenue of all channels, denoted by $\mbox{Rev}[\mathcal{R}]$, is
\begin{equation}
\label{eq:tcpa-ql}
\mbox{Rev}[\mathcal{R}]\ge\frac{(1-\varepsilon)(W_{\tiny \tcpa}^* + W_{\tiny \ql}^*)}{ 2 + 2\max\big \{1, \big \lceil \log \frac{T_{max}}{T_{min}}\big \rceil \big \}},
\end{equation}
where $W_{\tiny \tcpa}^*:=\sum_{k\in K}W_{\tiny \tcpa}^*(k)$ and $W_{\tiny \ql}^*:=\sum_{k\in K}W_{\tiny \ql}^*(k)$ denote the total contributions of $\tcpa$ and $\ql$ bidders to the liquid welfare of $x^*$ respectively.

Let $\rho(k,j)$ be as defined in Lemma~\ref{lem:budgeted-uniform}. Then, by Corollary~\ref{cor:min-rev-budg},
$$ \mbox{Rev}_k[\mathcal{R}] \geq \mathbf{E}_{\r\sim \mathcal{R}}\left[\frac{\sum_{j \in J^{E(\r)}_U} (1-\varepsilon)\rho(k,j) B_j}{2\max\big \{1, \big \lceil \log \frac{\beta_{max}}{\beta_{min}}\big \rceil \big \}}\right].
$$
Summing over all channels, we get 
\begin{equation}
\label{eq:nbc}    
\mbox{Rev}[\mathcal{R}] \geq \sum_k \mathbf{E}_{\r\sim \mathcal{R}}\left[\frac{\sum_{j \in J^{E(\r)}_U} (1-\varepsilon)\rho(k,j) B_j}{2\max\big \{1, \big \lceil \log \frac{\beta_{max}}{\beta_{min}}\big \rceil \big \}}\right] 
= \mathbf{E}_{\r\sim \mathcal{R}}\left[\frac{\sum_{j \in J^{E(\r)}_U} (1-\varepsilon)B_j}{2\max\big \{1, \big \lceil \log \frac{\beta_{max}}{\beta_{min}}\big \rceil \big \}}\right].
\end{equation}

Also, by item (1) of Lemma~\ref{lem:budgeted-uniform}, we have that
\begin{equation}
\label{eq:bc}
\mbox{Rev}[\mathcal{R}] \geq \mathbf{E}_{\r\sim \mathcal{R}}\left[\sum_{j \in J^{E(\r)}_C} B_j\right].
\end{equation}

Notice that 
$$Wel^* \leq W_{\tiny \tcpa}^* + W_{\tiny \ql}^* + \sum_{j \in J_{\tiny \budgeted}} B_j,$$
and then the theorem follows from Inequalities~\eqref{eq:tcpa-ql},~\eqref{eq:nbc} and~\eqref{eq:bc}.
\end{proof}

Combining Theorem~\ref{thm:rev-local} with Fact~\ref{fact:local-global}, we get the following corollary:
\begin{corollary}
\label{cor:rev-global}
For any $\varepsilon>0$, 
\begin{equation*}
RevG(Global) \geq \frac{1-\varepsilon}{3 + 2\max\big \{1, \big \lceil \log \frac{T_{max}}{T_{min}}\big \rceil \big \} +2\max\big \{1, \big \lceil \log \frac{\beta_{max}}{\beta_{min}}\big \rceil \big \}}.
\end{equation*}
\end{corollary}
\bigskip

Finally, we show that the above revenue guarantees in the local and global models are both tight up to a constant factor by constructing an example using the well-known "equal-revenue" trick.

\begin{proposition}\label{ex:revg-ub}
For the single-channel setting, there is an instance where $RevG(Global) = RevG(Local)=O(1/(\log(T_{max}/T_{min}) +\log( \beta_{max}/\beta_{min})))$.
\end{proposition}
\begin{proof}
Since there is only one channel, $RevG(Global) = RevG(Local)$.

Consider $2^{\ell}$ $\tcpa$ bidders with $\tcpa$s $1/2^{\ell}$ for $\ell=0, \ldots, w_1-1$, each interested in a unique impression with a value of $1$ (i.e. their value for every other impression is 0, and everyone else's value for their impression is 0). Similarly, there are $2^{\ell}$ $\budgeted$ bidders with budgets $1/2^{\ell}$ for $\ell=0, \ldots, w_2-1$, each interested in a unique impression with a value of $1$ (i.e. their value for every other impression is 0, and everyone else's value for their impression is 0). Optimal liquid welfare is $w_1 + w_2$ obtained by giving everyone their unique impression. The best uniform reserve price cannot get a revenue more than $4$. This shows that $RevG(Global) \leq 4 / (w_1+w_2) = 4 / (2 + \log \frac{T_{max}}{T_{min}} + \log \frac{\beta_{max}}{\beta_{min}})$.
\end{proof}

\subsection{Price of Anarchy}
In this subsection, we study how much total revenue the channels lose in the local model where they set their uniform reserve prices out of their own self-interest compared to the global model where they choose the reserve prices cooperatively. Specifically, we consider the standard notion -- price of anarchy $PoA$ (Definition~\ref{def:poa}).
First, we observe that the revenue guarantee from Theorem~\ref{thm:rev-local} immediately implies a lower bound for the $PoA$:
\begin{theorem}\label{lem:ineq-POA}
For any $\varepsilon>0$,
\begin{equation*}
     PoA \geq \frac{1-\varepsilon}{3 + 2\max\big \{1, \big \lceil \log \frac{T_{max}}{T_{min}}\big \rceil \big \} +2\max\big \{1, \big \lceil \log \frac{\beta_{max}}{\beta_{min}}\big \rceil \big \}}.
\end{equation*}
\end{theorem}
\begin{proof}
By definition of $PoA$ (Definition~\ref{def:poa}), $PoA=\frac{RevG(Local)}{RevG(Global)}$. By Fact~\ref{fact:local-global}, $RevG(Global)\le 1$. It follows that $PoA\ge RevG(Local)$, and then the proof finishes by applying Theorem~\ref{thm:rev-local}.
\end{proof}

Next, we show that the $PoA$ lower bound in Theorem~\ref{lem:ineq-POA} is tight (up to a constant factor).

\begin{theorem}\label{lem:tight-PoA}
There is an instance with two channels such that $PoA=O(1/(\log(T_{max}/T_{min}) +\log( \beta_{max}/\beta_{min})))$.
\end{theorem}
\paragraph{The high-level idea:} We first construct an ``equal-revenue'' instance (which consists of many $\tcpa$ bidders $J_1$ with geometrically decreasing $\tcpa$s, each interested in a unique impression owned by Channel $k_1$) as in the proof of Proposition~\ref{ex:revg-ub}. For this ``equal-revenue'' instance, Channel $k_1$ cannot simultaneously get good revenues from all the bidders in $J_1$ by setting a uniform reserve price.

Now the key idea is to introduce another Channel $k_2$ and another $\tcpa$ bidder $j_2\notin J_1$, such that Channel $k_2$ only owns one impression, for which only bidder $j_2$ has strictly positive value. Moreover, Bidder $j_2$ has a value for each impression $i$ in channel $k_1$, and Bidder $j_2$'s value for impression $i$ is carefully chosen to be proportional to the $\tcpa$ of the bidder in $J_1$ who is interested in impression $i$. Thus, if Bidder $j_2$ makes a uniform bid (in the cost-per-unit-value space), it results into non-uniform bids (in the cost space) for the impressions in Channel $k_1$, which are proportional to the $\tcpa$s of bidders in $J_1$. We can think of these non-uniform bids as non-uniform bidder-specific reserve prices for bidders in $J_1$, which are proportional to their $\tcpa$s. Thus, we are able to extract the full revenue from all the bidders in $J_1$ (similar to item (1) of Lemma~\ref{lem:tcpa-ql}).

Finally, we just need to argue the above idea can only be successfully applied in the global model but not in the local model. This is because in the local model, Channel $k_2$ sets a high reserve price for its sole impression in order to profit more from bidder $j_2$, and as a result, Bidder $j_2$ does not have enough ``slack'' to make a sufficiently high uniform bid to incur sufficiently high bidder-specific reserve prices for bidders in $J_1$.

The construction of the instance with $\budgeted$ bidders uses essentially the same idea as above. The full proof is provided in Appendix~\ref{app:sec5}.

%\ganote{Shall we send the detailed proof to the appendix?}

As a corollary of Theorem~\ref{lem:ineq-POA} and Theorem~\ref{lem:tight-PoA}, we have the following tight price of anarchy:
\begin{theorem}[Price of Anarchy]
\label{thm:poa-main}
$PoA=\Theta(1/(\log(T_{max}/T_{min}) +\log( \beta_{max}/\beta_{min})))$.
\end{theorem}

==> multi_channel (1)/05-pub-pricesII.tex <==
\section{Price of Anarchy with Publisher Reserves}\label{publisher-reserve}

This section studies the general version of the model where a publisher, owning impression $i$, sets a minimum price $p_i$ for the impression to be sold.\footnote{Recall that the price $p_i$ is also in the cost-per-unit-value space.} The main finding we obtain is that Theorem~\ref{thm:poa-main} dramatically depends on not having publisher prices. We show that with publisher prices and general channels,  $PoA = 0$ in the worst case (Theorem~\ref{th:general-publisher-model}). 

We then restrict our attention to an important subclass of instances where channels are {\em scaled} copy of each other. That is, channels share a set of a homogeneous set of impressions and differ on the revenue share each owns. In this context, we show that $PoA$ has non-trivial lower bound only if there is one bidder in the auction. In this case, $PoA = 1/|K|$, and hence, depends on the number of channels in the game in contrast to our results in Section~\ref{zero-publisher-reserve}. 


%We then explore an interes subclass when chan

%Our first result shows that in contrast with the case the no publisher prices, the $PoA = 0$ (Theorem~\ref{th:general-publisher-model}). 

%Key for this result is that there is an important heterogeneity in the publisher prices across the channels. For this reason we then restrict our attention for the cases where channels are {\em scaled} copy of each other. That is, channels have homogeneous set of impressions and only differ in the revenue share the obtain. In this context, we show that $PoA$ is finite only if there is one bidder in the auctions.

\subsection*{General Channels}

We now present the main result of the section for the general case when channels can have arbitrary asymmetries for the impressions they own with arbitrary publisher reserve prices.


\begin{theorem}\label{th:general-publisher-model}
If publishers can set arbitrary minimum prices on their impressions, then there is an instance for which $PoA = 0$.
\end{theorem}

\begin{proof}
Consider the following instance with two channels and one bidder who is a $\tcpa$ bidder with a target constraint $T=1$. Channel 1 has only one impression to sell. This impression does not have any publisher pricing constraint ($p_i=0$). Channel 2 has $q$ impressions to sell, each of these impressions has the same publisher pricing constraint $p_i = 1+ 1/q$. The bidder's valuation for all impressions is the same, i.e., $v_i = 1$ for all $i\in I$.

We assert that in the global model, it is optimal to set reserve prices equal to zero for both channels. Indeed, with no reserve prices, the bidder can purchase all impressions since she gets a value of $1+q$ for a total cost of $q\cdot (1+1/q) = 1+q$. This is the optimal solution for the global model as the total revenue is exactly the optimal liquid welfare.  

On the other hand, in the local model, it is a strictly dominant strategy for Channel 1 to set a uniform reserve $r_1=1$: if $r_1>1$, Channel 1 gets zero revenue. If $r_1\leq 1$, the bidder purchases its impression, which leads to a revenue of $r_1$. Thus, Channel 1 strictly prefers to set a reserve price of $r_1=1$. Because of $r_1=1$, the bidder cannot afford to buy any impression of Channel 2 since the cost of each impression is at least $1+1/q$. Thus, in this equilibrium, the bidder submits a uniform bid of $1$, gets only the impressions sold by Channel 1, and the global revenue is $1$.  

Therefore from this instance we have that $RevG(Local)/RevG(Global)\leq 1/(1+q)$. We conclude the proof by taking $q\to \infty$.
\end{proof}

The intuition behind the previous result comes from instances where some of the channels have high publisher prices relative to the bidder's $\tcpa$ targets while some other channels do not have publisher prices. In these instances, in the global model, channels benefit by keeping low reserve prices in the {\em cheap} channels (without publisher reserves) as they provide subsidy to the $\tcpa$ bidders to buy impressions from the {\em expensive} channels. However, when the cheap channels are myopic, they would like to raise their reserve prices to increase their local revenue. This local behavior negatively impacts the revenue of the expensive channels, which in turn, is negative for all channels.

Given that the reason for the previous negative $PoA$ result is the asymmetry of the publisher prices on the different channels, in what follows we restrict our $PoA$ analysis for a special subclass where channels are {\em scaled} versions of each other.
%\ganote{could say that each impression belongs to a channel with prob $\gamma_n$}\apnote{would channels set reserves before or after the realization of $\gg$?}

\subsection*{Scaled Channels}

%For simplicity of exposition, we now assume that each impression $i\in I$ is divisible. 
The scaled channels model consists of weights $\gg=(\gamma_1,\ldots,\gamma_k) \in \Delta([0,1]^K)$ \footnote{$\Delta([0,1]^K$ is the unit simplex in $\R^K$} so that Channel $k$ owns a fraction $\gamma_k$ of each impression $i\in I$.\footnote{For simplicity of the exposition we assume that impressions are divisible. A similar model with non-divisible impressions would assume that each impression $i$ is duplicated so that Channel $k$ owns a fraction $\gamma_k$ of those duplicates.}

%For the sake of exposition, we assume in the what follows that impressions are divisible. Then the scaled channels model consists of weights $\gg=(\gamma_1,\ldots,\gamma_k) \in \Delta([0,1]^K)$ \footnote{$\Delta([0,1]^K$ is the unit simplex in $\R^K$} so that Channel $k$ owns a fraction $\gamma_k$ of each impression $i\in I$. \footnote{A similar model with nondivisible impressions would assume that each impression $i$ is duplicated so that Channel $k$ owns a fraction $\gamma_k$ of those duplicates.}

 The first result shows that, surprisingly, so long as there are more than one bidder participating in the auctions, then $PoA = 0$ in the worst case.
 
 \begin{theorem}\label{th: scaled channels PoA=0}
 For the scaled channels models if there are two or more bidders participating in the auctions, then there is an instance for which $PoA = 0$.
 \end{theorem}
 
The instance we construct (deferred to Appendix~\ref{ap:sec-publisher}) consists of two channels and two $\tcpa$ bidders. The idea of the instance is that the main source of revenue for the channels comes from Bidder 1 buying the expensive impressions, those with high publisher reserve price. Bidder 1 needs enough slack to be able to purchase those expensive impressions. Thus, Bidder 1 needs to buy enough cheap impressions. However, the cheap impressions may have a high price if Bidder 2 sets a high bid. Bidder 2 can only set a high bid if, instead, it has enough slack from (other) cheap impressions. The crux of the argument is that, in the global model, by setting a sufficiently high reserve price, the channels can avoid Bidder 2 to have enough slack. This, in turn, allows Bidder $1$ to have slack to buy the expensive impressions. On the contrary, for the local models, there is an equilibrium where both channels set a low reserve. This prevents Bidder 1 to buy expensive impressions because Bidder 2 is setting a high bid and removing Bidder 1's slack.

As a corollary of this instance, we show that in the autobidding framework setting a high reserve price like in the global model not only increases revenue but also increases the welfare. This contrasts with the classic profit-maximizing framework where there is a negative correlation between high reserve prices and welfare.

%The $\tcpa$ bidder 2 is an ``unwanted bidder'' for the platform because if bidder $2$ has enough slack (by buying cheap impressions) it prices the cheap impressions of bidder 1 high enough. This removes bidder 1's slack and, hence, bidder 1 cannot purchase the impressions that have high publisher prices. In the global model this issue is avoided by setting a high reserve price that removes the slack of bidder 2. In the local model, instead, there is an equilibrium where channels don't set a reserve price which is why the local model has a low performance compared to the global model.

%\Andres{Do we want to keep this?: A second interesting feature we observe in this instance is that when setting a high reserve prices not only the revenue is larger but also the liquid welfare. This contrasts with the classic profit-maximizing framework where there is a negative correlation between reserve prices and welfare.}

We finish this section by showing that for the case of only one bidder participating across all channels the $PoA$ is always strictly positive (for pure-strategy equilibria).

\begin{theorem}\label{poa: 1/k}
If there is only a single bidder, then for pure-strategy equilibria we have that $PoA =\frac {1}{ |K|}$, where $|K|$ is the number of channels in the game.
\end{theorem}

We defer the proof to Appendix~\ref{ap:sec-publisher}. We note that in contrast to the results of Section~\ref{zero-publisher-reserve} where the $PoA$ is independent of the number of channels, in the setting with publisher reserves, the $PoA$ directly depends of the number of channels.

==> multi_channel (1)/07-Further-discussions.tex <==
\section{Further Discussion}\label{sec: further-discussions}
In this paper, we have established tight bounds on \emph{revenue} guarantees and Price of Anarchy when the reserve prices are set in the \emph{cost-per-unit-value} space. Two natural follow-up questions are:
\begin{quote}
    \begin{itemize}
        \item Can we obtain similar bounds for \emph{welfare} of the bidders?
        \item What are the revenue guarantees if the channels set reserve prices in the \emph{cost-per-impression} space?
    \end{itemize}
\end{quote}

We briefly discuss how to extend some of our results to answer these questions. We defer the details to the full paper.
%Answering these questions are interesting future directions. In the following, we want to mention the implications of our results in this paper for these two questions:
\subsection*{Bounds for Welfare}
Most of our revenue and Price of Anarchy results carry over to {\em welfare}. In particular for the setting without publisher reserves, we can get bounds similar to the the revenue bounds in Theorem~\ref{thm:rev-local} and Proposition~\ref{ex:revg-ub} and the Price of Anarchy bound in Theorem~\ref{thm:poa-main} for welfare (see Appendix~\ref{app:welfare} for a proof sketch). Many of the results in the setting without publisher reserves also carry over to welfare. We defer the details to the full paper.

We also observe an interesting phenomena -- in contrast to the quasi-linear setting, using a higher reserve price can sometimes increase the welfare (see the discussion after Theorem~\ref{th: scaled channels PoA=0}).

\subsection*{Uniform cost-per-impression reserve prices}
 We can obtain a revenue guarantee analogous to Theorem~\ref{thm:rev-local} when channels set uniform cost-per-impression reserve prices (i.e., value-independent and the same for all bidders and impressions). We can do this by adapting the bucketization arguments in Section~\ref{zero-publisher-reserve} to bucketize $T_j v_{j,i}$ instead of $T_j$ for $\tcpa$ bidders, bucketize $v_{j,i}$ for Quasi-linear bidders, and bucketize $\beta_j v_{j,i}$ instead of $\beta_j$ for $\budgeted$ bidders.
%    \Junyao{This is vague -- make changes or remove if you want}
%    \ganote{I think these are correct -- the key observation is that observation 4 applies on a per impression basis. Then you essentially need to set beta_j v_ij as the final reserve price for imp ij. So you can bucketize beta_j v_ij, rather than beta_j. }


==> multi_channel (1)/header.tex <==
\usepackage{amsmath,amsfonts,amsthm}
\usepackage{thmtools} % Used to restate lemmas without new introducing new numbers.
%\usepackage{hyperref}
\usepackage{xcolor}
%\usepackage{times}
\usepackage{amssymb}
\usepackage{bm}
\usepackage{xspace}
%\usepackage[backref,pageanchor=true,plainpages=false, pdfpagelabels, bookmarks,bookmarksnumbered,
%pdfborder=0 0 0,  %removes outlines around hyper links in online display
%]{hyperref}
\usepackage{mathtools}
\usepackage{hyperref}
\usepackage{nicefrac}
\usepackage{natbib}

\usepackage{comment}



%\usepackage{enumitem}
%\usepackage[ruled,vlined]{algorithm2e}
%\usepackage{stmaryrd}

%\sloppy
%\frenchspacing

%\usepackage[margin=1in]{geometry}



\newtheorem{theorem}{Theorem}
\newtheorem{lemma}{Lemma}
\newtheorem{proposition}{Proposition}
\newtheorem{claim}{Claim}
\newtheorem{corollary}{Corollary}
\newtheorem{definition}{Definition}
\newtheorem{observation}{Observation}
\newtheorem{task}{Task}
\newtheorem{conjecture}{Conjecture}
\newtheorem{fact}{Fact}
\newtheorem{example}{Example}
%\renewcommand\thefactl{\Alph{factl}}
%\newtheorem{question}{Question}
\newtheorem{remark}{Remark}
\newtheorem{assumption}{Assumption}

\DeclareMathOperator*{\argmax}{arg\,max}
\DeclareMathOperator*{\argmin}{arg\,min}

\def\N{\mathbb{N}}
\def\Q{\mathbb{Q}}
\def\R{\mathbb{R}}
\def \P{\mathbb{P}}

\newcommand{\E}{\mathbb{E}}
\renewcommand{\u}{\tilde{u}}
\newcommand{\U}{\tilde{U}}
\newcommand{\X}{\mathcal{X}}
%\newcommand{\ggz}{\gg}
\renewcommand{\gg}{\bm{\gamma}}
\renewcommand{\k}{\hat{k}}


\newcommand{\tcpa}{{ \mbox{tCPA} }}
\newcommand{\ql}{{ \mbox{QL} }}
\newcommand{\budgeted}{{ \mbox{Budgeted} }}
\newcommand{\budget}{{ \mbox{B} }}
\newcommand{\PPAD}{{\texttt{PPAD}}}


\def\mK{{\bm{K}}}
\def\mQ{{\bm{Q}}}
\def\mV{{\bm{V}}}
\def\mX{{\bm{X}}}
\def\mY{{\bm{Y}}}
\def\mZ{{\bm{Z}}}


\def\vzero{{\bm{0}}}
\def\vtheta{{\bm{\theta}}}
\def\b{{\bm{b}}}
\def\r{{\bm{r}}}
\def \x {{\bm{x}}}
\def\v{{\bm{v}}}
\def\va{{\bm{a}}}
\def\vi{{\bm{i}}}
\def\vj{{\bm{j}}}
\def\vk{{\bm{k}}}
\def\vp{{\bm{p}}}
\def\vq{{\bm{q}}}
\def\vr{{\bm{r}}}
\def\vs{{\bm{s}}}
\def\vt{{\bm{t}}}
\def\vu{{\bm{u}}}
\def\vv{{\bm{v}}}
\def\vw{{\bm{w}}}
\def\x{{\bm{x}}}
\def\vy{{\bm{y}}}
\def\vz{{\bm{z}}}
\def \cC {\mathcal{C}}
\def \cD {\mathcal{D}}
\def \cG {\mathcal{G}}
\def \cI {\mathcal{I}}
\def \cT {\mathcal{T}}
\def \eps {\varepsilon}


\newcommand{\lu}{\underline{\phantom{A}}}


\DeclarePairedDelimiter{\ceil}{\lceil}{\rceil}
\DeclarePairedDelimiter{\floor}{\lfloor}{\rfloor}
\DeclarePairedDelimiter{\abs}{\lvert}{\rvert}
\DeclarePairedDelimiter{\norm}{\|}{\|}
\DeclarePairedDelimiter{\braket}{ \left \langle}{ \right \rangle}
\DeclarePairedDelimiter{\set}{ \{ }{ \} }
\newcommand{\bkt}[2]{\left \langle #1, #2 \right \rangle}
%\newcommand{\eps}{\varepsilon}
\newcommand{\NPHard}{\textsc{NP}-Hard\xspace}

\newcommand{\OPT}{\textsc{OPT}}

% Uncomment the line below to turn off all notes.
%\newcommand{\NOCOMMENT}{}

\ifdefined\NOCOMMENT
    \newcommand{\ganote}[1]{}
    \newcommand{\apnote}[1]{}
    \newcommand{\jznote}[1]{}
    
\else
    \newcounter{note}[section]
    \renewcommand{\thenote}{\thesection.\arabic{note}}

    
\newcommand{\apnote}[1]{\refstepcounter{note}\textcolor{blue}{$\ll${\bf Andres~\thenote:} {\sf #1}$\ggg$\marginpar{\tiny\bf AP~\thenote}}}
    
\newcommand{\ganote}[1]{\refstepcounter{note}\textcolor{blue}{$\ll${\bf Gagan~\thenote:} {\sf #1}$\ggg$\marginpar{\tiny\bf GA~\thenote}}}
    
\newcommand{\jznote}[1]{\refstepcounter{note}\textcolor{brown}{$\ll${\bf Junyao~\thenote:} {\sf #1}$\ggg$\marginpar{\tiny\bf JZ~\thenote}}}
